Are the Values of LLMs Structurally Aligned with Humans? A Causal Perspective

As large language models (LLMs) become increasingly integrated into critical applications, aligning their behavior with human values presents significant challenges. Current methods, such as Reinforcement Learning from Human Feedback (RLHF), typically focus on a limited set of coarse-grained values and are resource-intensive. Moreover, the correlations between these values remain implicit, leading to unclear explanations for value-steering outcomes. Our work argues that a latent causal value graph underlies the value dimensions of LLMs and that, despite alignment training, this structure remains significantly different from human value systems. We leverage these causal value graphs to guide two lightweight value-steering methods: role-based prompting and sparse autoencoder (SAE) steering, effectively mitigating unexpected side effects. Furthermore, SAE provides a more fine-grained approach to value steering. Experiments on Gemma-2B-IT and Llama3-8B-IT demonstrate the effectiveness and controllability of our methods.

==> bak.tex <==
\begin{table*}[ht]
\caption{Value steering using SAE features for the Gemma-2B-IT model. Expected stimulated values are highlighted in red, along with their actual success rate during testing. Expected suppressed values are marked in Purple. Maintained values are shown in gray. Light red indicates values that are expected to be at least not suppressed, while light purple represents values that are expected to be at least not stimulated. Blank cells correspond to uncontrollable values. The bottom of the table indicates the count of each of the six expected categories and their average success rates.}
\label{table: sae-steering-gemma}
\begin{center}
\scalebox{0.5}{\begin{tabular}{c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c}
\toprule
Value & \rotatebox{90}{\bf Achievement} & \rotatebox{90}{\bf Aesthetic} & \rotatebox{90}{\bf Anxiety Disorder} & \rotatebox{90}{\bf Breadth of Interest} & \rotatebox{90}{\bf Economic} & \rotatebox{90}{\bf Empathy} & \rotatebox{90}{\bf Organization} & \rotatebox{90}{\bf Political} & \rotatebox{90}{\bf Positive coping} & \rotatebox{90}{\bf Religious} & \rotatebox{90}{\bf Resilience} & \rotatebox{90}{\bf Social} & \rotatebox{90}{\bf Social Complexity} & \rotatebox{90}{\bf Social Cynicism} & \rotatebox{90}{\bf Theoretical} & \rotatebox{90}{\bf Uncertainty Avoidance} & \rotatebox{90}{\bf Understanding} &\rotatebox{90} {\bf STIMULATE} & \rotatebox{90} {\bf SUPPRESS} & \rotatebox{90} {\bf NON-SUPPRESS}& \rotatebox{90} {\bf NON-STIMULATE} & \rotatebox{90} {\bf MAINTAIN} & \rotatebox{90} {\bf UNCONTROLLED} \\
\hline
\small 428.0 & \colorbox{blue!20}{0.60} & \colorbox{blue!20}{0.80} & \colorbox{red!20}{0.68} & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.96} & - & \colorbox{red!20}{0.88} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.80} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.80} & \colorbox{blue!20}{0.60} & \colorbox{gray!20}{0.40} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.76} & \colorbox{blue!20}{0.88}  & 0(nan) & 0(nan) & 8(0.88) & 7(0.794) & 1(0.4) & 1 \ \\
\small 1025.0 & \colorbox{blue!20}{0.80} & \colorbox{blue!20}{0.88} & - & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.92} & \colorbox{blue!20}{0.88} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.80} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.96} & \colorbox{gray!20}{0.88} & \colorbox{blue!20}{0.84} & \colorbox{gray!20}{0.80} & \colorbox{gray!20}{0.92} & \colorbox{red!20}{0.60} & \colorbox{red!20}{0.84}  & 0(nan) & 0(nan) & 7(0.874) & 6(0.887) & 3(0.867) & 1 \ \\
\small 1312.0 & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.76} & \colorbox{red!50}{0.80} & \colorbox{blue!50}{0.04} & \colorbox{red!20}{0.92} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.48} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.72} & \colorbox{gray!20}{0.08} & \colorbox{blue!50}{0.20} & \colorbox{red!20}{0.08} & \colorbox{red!20}{0.96} & \colorbox{red!50}{0.48} & \colorbox{blue!20}{0.68}  & 2(0.64) & 2(0.12) & 7(0.743) & 5(0.856) & 1(0.08) & 0 \ \\
\small 1341.0 & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.96} & - & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.92} & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.96} & - & \colorbox{red!20}{0.64} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.92} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.92} & \colorbox{gray!20}{0.88} & \colorbox{red!20}{0.88} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.92}  & 0(nan) & 0(nan) & 7(0.886) & 7(0.949) & 1(0.88) & 2 \ \\
\small 1975.0 & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.64} & - & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.84} & \colorbox{blue!20}{0.76} & \colorbox{red!20}{0.88} & \colorbox{blue!20}{0.96} & \colorbox{red!50}{0.44} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.36} & \colorbox{red!20}{0.92} & \colorbox{red!20}{0.96} & \colorbox{gray!20}{0.48} & \colorbox{red!20}{0.76} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.88}  & 1(0.44) & 0(nan) & 6(0.807) & 8(0.865) & 1(0.48) & 1 \ \\
\small 2221.0 & \colorbox{red!20}{0.88} & \colorbox{blue!20}{0.96} & - & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{0.80} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.92} & \colorbox{gray!20}{0.84} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.28} & \colorbox{gray!20}{0.80} & - & \colorbox{red!20}{0.48}  & 0(nan) & 0(nan) & 4(0.66) & 9(0.956) & 2(0.82) & 2 \ \\
\small 2965.0 & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.96} & - & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.84} & - & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.92} & \colorbox{red!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{1.00} & \colorbox{gray!20}{1.00} & \colorbox{red!20}{0.28} & \colorbox{gray!20}{0.76} & \colorbox{gray!20}{0.92} & \colorbox{red!20}{0.88} & \colorbox{gray!20}{0.96}  & 0(nan) & 0(nan) & 8(0.85) & 3(0.987) & 4(0.91) & 2 \ \\
\small 3183.0 & \colorbox{blue!20}{0.96} & - & \colorbox{red!50}{0.88} & \colorbox{blue!20}{0.52} & - & \colorbox{blue!20}{0.80} & - & - & - & \colorbox{red!50}{0.00} & \colorbox{red!20}{0.44} & - & \colorbox{blue!20}{0.48} & \colorbox{red!20}{0.96} & \colorbox{red!50}{0.80} & \colorbox{red!50}{1.00} & \colorbox{blue!20}{0.52}  & 4(0.67) & 0(nan) & 2(0.7) & 5(0.656) & 0(nan) & 6 \ \\
\small 3402.0 & \colorbox{red!20}{0.84} & \colorbox{blue!20}{0.92} & - & \colorbox{blue!20}{0.60} & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.88} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{1.00} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.72} & \colorbox{blue!20}{0.92} & \colorbox{gray!20}{0.80} & \colorbox{blue!20}{0.96} & \colorbox{gray!20}{0.32} & \colorbox{gray!20}{1.00} & \colorbox{red!20}{0.64} & \colorbox{red!20}{0.92}  & 0(nan) & 0(nan) & 6(0.853) & 7(0.886) & 3(0.707) & 1 \ \\
\small 4752.0 & \colorbox{blue!20}{0.92} & \colorbox{blue!20}{0.52} & \colorbox{red!20}{0.40} & \colorbox{blue!20}{0.76} & \colorbox{red!20}{0.96} & - & - & - & \colorbox{red!20}{0.72} & \colorbox{blue!20}{0.92} & \colorbox{blue!50}{0.68} & \colorbox{red!20}{0.92} & \colorbox{blue!50}{0.96} & \colorbox{blue!50}{0.96} & \colorbox{red!20}{0.96} & - & \colorbox{red!20}{0.76}  & 0(nan) & 3(0.867) & 6(0.787) & 4(0.78) & 0(nan) & 4 \ \\
\small 6188.0 & \colorbox{red!20}{0.84} & \colorbox{blue!20}{0.84} & - & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.68} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.76} & \colorbox{red!20}{0.60} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.72} & \colorbox{gray!20}{0.36} & \colorbox{gray!20}{0.84} & \colorbox{red!20}{0.64} & \colorbox{red!20}{0.84}  & 0(nan) & 0(nan) & 8(0.795) & 6(0.907) & 2(0.6) & 1 \ \\
\small 6216.0 & \colorbox{red!20}{0.92} & \colorbox{blue!20}{0.92} & - & \colorbox{blue!50}{0.08} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.88} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.92} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{1.00} & \colorbox{gray!20}{0.76} & \colorbox{blue!20}{0.64} & \colorbox{red!20}{0.28} & \colorbox{gray!20}{0.92} & \colorbox{red!20}{1.00} & \colorbox{gray!20}{0.76}  & 0(nan) & 1(0.08) & 7(0.863) & 5(0.88) & 3(0.813) & 1 \ \\
\small 6619.0 & - & \colorbox{blue!20}{0.48} & - & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.84} & \colorbox{blue!20}{0.88} & \colorbox{red!20}{0.84} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.88} & - & \colorbox{red!20}{0.40} & \colorbox{gray!20}{0.88} & \colorbox{red!20}{0.60} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.12} & \colorbox{red!20}{0.88} & \colorbox{red!20}{0.60}  & 0(nan) & 0(nan) & 8(0.75) & 5(0.672) & 1(0.88) & 3 \ \\
\small 6884.0 & - & \colorbox{blue!20}{0.52} & - & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.84} & - & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.72} & - & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.88} & \colorbox{red!20}{0.68} & \colorbox{red!20}{0.68}  & 0(nan) & 0(nan) & 5(0.784) & 8(0.9) & 0(nan) & 4 \ \\
\small 7502.0 & \colorbox{blue!20}{0.80} & \colorbox{blue!20}{0.92} & - & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.96} & - & \colorbox{red!20}{0.92} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.92} & \colorbox{gray!20}{0.88} & \colorbox{blue!20}{1.00} & \colorbox{gray!20}{0.24} & \colorbox{gray!20}{0.96} & \colorbox{red!20}{0.88} & \colorbox{gray!20}{0.72}  & 0(nan) & 0(nan) & 5(0.944) & 6(0.933) & 4(0.7) & 2 \ \\
\small 8387.0 & - & - & \colorbox{blue!20}{0.40} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.88} & \colorbox{red!20}{1.00} & - & \colorbox{red!20}{0.80} & \colorbox{blue!20}{1.00} & - & \colorbox{red!20}{0.32} & \colorbox{blue!20}{0.44} & \colorbox{blue!20}{0.76} & \colorbox{red!20}{0.36} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.76}  & 0(nan) & 0(nan) & 8(0.76) & 5(0.712) & 0(nan) & 4 \ \\
\small 10096.0 & - & - & - & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.88} & \colorbox{red!20}{0.64} & - & \colorbox{blue!20}{0.92} & - & - & - & \colorbox{blue!20}{0.76} & \colorbox{gray!20}{0.48} & \colorbox{red!20}{0.84} & - & \colorbox{red!20}{0.84}  & 0(nan) & 0(nan) & 6(0.86) & 2(0.84) & 1(0.48) & 8 \ \\
\small 10454.0 & \colorbox{red!20}{0.84} & \colorbox{blue!20}{0.64} & - & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.88} & \colorbox{blue!20}{0.92} & \colorbox{red!20}{0.88} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.80} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.96} & \colorbox{gray!20}{0.88} & \colorbox{blue!20}{1.00} & \colorbox{gray!20}{0.28} & \colorbox{gray!20}{0.96} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.72}  & 0(nan) & 0(nan) & 6(0.847) & 7(0.92) & 3(0.707) & 1 \ \\
\small 10605.0 & \colorbox{blue!20}{0.80} & \colorbox{blue!20}{0.84} & - & \colorbox{blue!20}{0.68} & \colorbox{blue!20}{0.76} & \colorbox{red!20}{0.36} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.72} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.92} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.68} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.84}  & 0(nan) & 0(nan) & 7(0.794) & 9(0.876) & 0(nan) & 1 \ \\
\small 11712.0 & \colorbox{red!20}{0.76} & \colorbox{red!20}{0.96} & - & \colorbox{gray!20}{0.72} & \colorbox{blue!20}{0.56} & \colorbox{blue!20}{0.68} & \colorbox{red!20}{0.92} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.68} & \colorbox{red!20}{0.60} & \colorbox{blue!20}{0.96} & \colorbox{gray!20}{0.96} & \colorbox{blue!20}{1.00} & \colorbox{gray!20}{0.40} & \colorbox{red!20}{0.52} & \colorbox{red!20}{0.84} & \colorbox{red!20}{0.64}  & 0(nan) & 0(nan) & 8(0.74) & 5(0.84) & 3(0.693) & 1 \ \\
\small 12703.0 & \colorbox{red!20}{0.64} & \colorbox{red!20}{1.00} & - & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.84} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.88} & \colorbox{red!20}{1.00} & \colorbox{gray!20}{0.76} & \colorbox{blue!20}{0.72} & \colorbox{red!20}{0.36} & \colorbox{gray!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.76}  & 0(nan) & 0(nan) & 8(0.83) & 6(0.9) & 2(0.86) & 1 \ \\
\small 14049.0 & - & \colorbox{blue!20}{0.52} & - & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{0.68} & - & \colorbox{blue!50}{0.60} & \colorbox{red!20}{0.80} & \colorbox{red!20}{0.92} & - & \colorbox{blue!20}{0.84} & \colorbox{red!20}{1.00} & - & \colorbox{red!20}{0.96} & \colorbox{red!20}{0.52} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.84}  & 0(nan) & 1(0.6) & 6(0.86) & 5(0.776) & 0(nan) & 5 \ \\
\small 14185.0 & - & \colorbox{red!20}{0.64} & - & \colorbox{red!20}{0.76} & \colorbox{red!20}{1.00} & \colorbox{blue!20}{0.48} & - & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.60} & \colorbox{blue!20}{1.00} & \colorbox{blue!20}{0.88} & \colorbox{red!20}{0.88} & \colorbox{blue!20}{0.96} & \colorbox{red!20}{0.92} & \colorbox{red!20}{0.84} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.44}  & 0(nan) & 0(nan) & 9(0.844) & 5(0.752) & 0(nan) & 3 \ \\
\small 14351.0 & \colorbox{red!20}{0.96} & \colorbox{blue!20}{1.00} & - & \colorbox{blue!20}{0.96} & \colorbox{blue!20}{0.76} & \colorbox{blue!20}{1.00} & \colorbox{red!20}{0.96} & \colorbox{red!20}{1.00} & \colorbox{red!20}{1.00} & \colorbox{red!20}{0.96} & \colorbox{blue!20}{0.96} & \colorbox{gray!20}{1.00} & \colorbox{blue!20}{0.88} & \colorbox{gray!20}{0.32} & \colorbox{gray!20}{0.96} & \colorbox{red!20}{0.88} & \colorbox{gray!20}{0.80}  & 0(nan) & 0(nan) & 6(0.96) & 6(0.927) & 4(0.77) & 1 \ \\
 \midrule
 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

\begin{table*}[ht]
\caption{Value steering using SAE features for the Gemma-2B-IT model. Stimulated values are in red and suppressed values are marked in Purple. Maintained values are shown in gray. Light red indicates values that are expected to be at least not suppressed, while light purple represents values that are expected to be at least not stimulated. Blank cells correspond to uncontrollable values. The bottom of the table indicates the count of each of the six expected categories and their average success rates.}
\label{table: sae-steering-gemma}
\begin{center}
\scalebox{0.5}{\begin{tabular}{c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c@{\hspace{1.5pt}}|c}
\toprule
\rotatebox{90}{Value} & \rotatebox{90}{\bf Achievement} & \rotatebox{90}{\bf Aesthetic} & \rotatebox{90}{\bf Anxiety Disorder} & \rotatebox{90}{\bf Breadth of Interest} & \rotatebox{90}{\bf Economic} & \rotatebox{90}{\bf Empathy} & \rotatebox{90}{\bf Organization} & \rotatebox{90}{\bf Political} & \rotatebox{90}{\bf Positive coping} & \rotatebox{90}{\bf Religious} & \rotatebox{90}{\bf Resilience} & \rotatebox{90}{\bf Social} & \rotatebox{90}{\bf Social Complexity} & \rotatebox{90}{\bf Social Cynicism} & \rotatebox{90}{\bf Theoretical} & \rotatebox{90}{\bf Uncertainty Avoidance} & \rotatebox{90}{\bf Understanding}&\rotatebox{90}{\bf AVG} \\
\hline
\small 428 & \colorbox[rgb]{0.77,0.81,0.62}{0.90} & \colorbox[rgb]{0.77,0.85,0.65}{0.96} & \colorbox[rgb]{0.81,0.54,0.44}{0.90} & \colorbox[rgb]{0.68,0.97,0.66}{0.94} & \colorbox[rgb]{0.96,0.59,0.57}{1.00} & \colorbox[rgb]{0.71,0.77,0.55}{0.60} & \colorbox[rgb]{0.93,0.42,0.4}{0.57} & \colorbox[rgb]{0.88,0.51,0.45}{0.65} & \colorbox[rgb]{0.92,0.7,0.65}{0.98} & \colorbox[rgb]{0.78,0.8,0.62}{0.92} & \colorbox[rgb]{0.81,0.78,0.63}{0.97} & \colorbox[rgb]{0.72,0.97,0.7}{0.91} & \colorbox[rgb]{0.69,0.83,0.57}{0.87} & \colorbox[rgb]{1.0,0.9,0.9}{0.72} & \colorbox[rgb]{0.94,0.89,0.84}{0.99} & \colorbox[rgb]{0.93,0.55,0.51}{0.89} & \colorbox[rgb]{0.75,0.94,0.71}{0.99}  & 0.87 \\
\small 1025 & \colorbox[rgb]{0.78,0.8,0.62}{0.97} & \colorbox[rgb]{0.75,0.96,0.72}{0.96} & \colorbox[rgb]{0.77,0.64,0.49}{0.97} & \colorbox[rgb]{0.7,0.93,0.65}{0.98} & \colorbox[rgb]{0.85,0.85,0.72}{0.99} & \colorbox[rgb]{0.73,0.87,0.64}{1.00} & \colorbox[rgb]{0.86,0.67,0.58}{0.85} & \colorbox[rgb]{0.74,0.9,0.67}{0.97} & \colorbox[rgb]{0.99,0.7,0.69}{0.75} & \colorbox[rgb]{0.84,0.96,0.81}{0.98} & \colorbox[rgb]{0.9,0.77,0.69}{0.96} & \colorbox[rgb]{0.96,0.99,0.95}{0.99} & \colorbox[rgb]{0.73,0.85,0.62}{0.89} & \colorbox[rgb]{0.95,0.96,0.91}{0.99} & \colorbox[rgb]{0.91,1.0,0.91}{1.00} & \colorbox[rgb]{0.94,0.7,0.66}{0.80} & \colorbox[rgb]{0.81,0.99,0.8}{0.99}  & 0.94 \\
\small 1312 & \colorbox[rgb]{0.74,0.86,0.64}{0.96} & \colorbox[rgb]{0.86,0.79,0.68}{0.96} & \colorbox[rgb]{0.85,0.23,0.19}{0.99} & \colorbox[rgb]{0.29,1.0,0.29}{0.41} & \colorbox[rgb]{0.87,0.77,0.67}{0.99} & \colorbox[rgb]{0.53,0.84,0.45}{0.78} & \colorbox[rgb]{0.73,0.91,0.67}{0.94} & \colorbox[rgb]{0.81,0.77,0.62}{0.91} & \colorbox[rgb]{0.94,0.74,0.7}{0.65} & \colorbox[rgb]{0.96,0.44,0.43}{0.66} & \colorbox[rgb]{0.67,0.85,0.57}{0.88} & \colorbox[rgb]{0.95,0.96,0.91}{0.18} & \colorbox[rgb]{0.25,0.93,0.23}{0.47} & \colorbox[rgb]{0.99,0.48,0.48}{0.08} & \colorbox[rgb]{0.94,0.66,0.62}{0.87} & \colorbox[rgb]{1.0,0.29,0.29}{0.93} & \colorbox[rgb]{0.77,0.99,0.76}{0.88}  & 0.74 \\
\small 1341 & \colorbox[rgb]{0.76,0.8,0.61}{0.97} & \colorbox[rgb]{0.83,0.73,0.61}{0.92} & \colorbox[rgb]{0.72,0.59,0.43}{0.99} & \colorbox[rgb]{0.64,0.93,0.6}{0.91} & \colorbox[rgb]{0.87,0.81,0.71}{0.80} & \colorbox[rgb]{0.75,0.87,0.65}{0.90} & \colorbox[rgb]{0.69,0.86,0.6}{0.86} & \colorbox[rgb]{0.58,0.79,0.46}{0.72} & \colorbox[rgb]{0.95,0.61,0.58}{0.79} & \colorbox[rgb]{0.54,0.9,0.49}{0.98} & \colorbox[rgb]{0.97,0.61,0.59}{0.83} & \colorbox[rgb]{0.75,0.88,0.66}{0.94} & \colorbox[rgb]{0.48,0.93,0.45}{0.99} & \colorbox[rgb]{0.9,1.0,0.9}{0.99} & \colorbox[rgb]{0.9,0.83,0.75}{0.98} & \colorbox[rgb]{0.86,0.82,0.71}{0.93} & \colorbox[rgb]{0.92,0.81,0.75}{0.62}  & 0.89 \\
\small 1975 & \colorbox[rgb]{0.77,0.89,0.69}{0.88} & \colorbox[rgb]{0.59,0.82,0.49}{0.81} & \colorbox[rgb]{0.65,0.75,0.49}{0.84} & \colorbox[rgb]{0.76,0.95,0.72}{0.96} & \colorbox[rgb]{0.79,0.84,0.66}{0.92} & \colorbox[rgb]{0.36,0.98,0.36}{0.65} & \colorbox[rgb]{0.85,0.53,0.45}{0.68} & \colorbox[rgb]{0.61,0.88,0.54}{0.78} & \colorbox[rgb]{0.89,0.33,0.3}{0.92} & \colorbox[rgb]{0.65,0.82,0.53}{0.66} & \colorbox[rgb]{0.82,0.88,0.72}{0.68} & \colorbox[rgb]{0.84,0.98,0.82}{0.99} & \colorbox[rgb]{0.9,0.79,0.71}{0.74} & \colorbox[rgb]{0.98,0.89,0.87}{0.83} & \colorbox[rgb]{0.81,0.99,0.8}{0.99} & \colorbox[rgb]{0.89,0.75,0.67}{0.99} & \colorbox[rgb]{0.71,0.97,0.69}{0.99}  & 0.84 \\
\small 2221 & \colorbox[rgb]{0.82,0.78,0.64}{0.91} & \colorbox[rgb]{0.71,0.9,0.64}{0.95} & \colorbox[rgb]{0.76,0.73,0.56}{0.95} & \colorbox[rgb]{0.62,0.97,0.6}{0.99} & \colorbox[rgb]{0.72,0.8,0.58}{0.99} & \colorbox[rgb]{0.69,0.88,0.61}{0.50} & \colorbox[rgb]{0.61,0.8,0.49}{0.69} & \colorbox[rgb]{0.71,0.9,0.64}{0.91} & \colorbox[rgb]{0.92,0.71,0.65}{0.84} & \colorbox[rgb]{0.7,0.94,0.66}{0.93} & \colorbox[rgb]{0.49,0.98,0.48}{0.72} & \colorbox[rgb]{0.93,0.97,0.9}{1.00} & \colorbox[rgb]{0.59,0.9,0.53}{0.86} & \colorbox[rgb]{0.8,0.96,0.77}{0.55} & \colorbox[rgb]{0.96,0.96,0.92}{0.99} & \colorbox[rgb]{0.75,0.77,0.58}{0.97} & \colorbox[rgb]{0.91,0.87,0.79}{0.59}  & 0.84 \\
\small 2965 & \colorbox[rgb]{0.91,0.86,0.78}{1.00} & \colorbox[rgb]{0.73,0.98,0.72}{0.94} & \colorbox[rgb]{0.72,0.74,0.53}{0.89} & \colorbox[rgb]{0.63,1.0,0.63}{0.87} & \colorbox[rgb]{0.84,0.83,0.7}{1.00} & \colorbox[rgb]{0.67,0.78,0.53}{0.97} & \colorbox[rgb]{0.91,0.8,0.73}{0.96} & \colorbox[rgb]{0.88,0.89,0.78}{0.99} & \colorbox[rgb]{0.96,0.77,0.74}{0.48} & \colorbox[rgb]{0.87,0.96,0.84}{0.99} & \colorbox[rgb]{0.77,0.99,0.76}{0.96} & \colorbox[rgb]{0.97,0.9,0.87}{0.99} & \colorbox[rgb]{0.86,0.87,0.75}{0.37} & \colorbox[rgb]{0.86,0.99,0.85}{0.99} & \colorbox[rgb]{0.99,0.92,0.91}{1.00} & \colorbox[rgb]{0.83,0.81,0.67}{0.99} & \colorbox[rgb]{0.86,0.99,0.85}{0.99}  & 0.90 \\
\small 3183 & \colorbox[rgb]{0.4,0.81,0.33}{0.95} & \colorbox[rgb]{0.74,0.42,0.31}{0.67} & \colorbox[rgb]{0.86,0.31,0.27}{0.97} & \colorbox[rgb]{0.5,0.84,0.42}{0.80} & \colorbox[rgb]{0.53,0.75,0.4}{0.60} & \colorbox[rgb]{0.39,0.8,0.31}{0.97} & \colorbox[rgb]{0.57,0.78,0.45}{0.75} & \colorbox[rgb]{0.63,0.6,0.38}{0.74} & \colorbox[rgb]{0.67,0.67,0.45}{0.88} & \colorbox[rgb]{0.92,0.24,0.22}{0.16} & \colorbox[rgb]{0.93,0.54,0.51}{0.53} & \colorbox[rgb]{0.54,0.72,0.39}{0.88} & \colorbox[rgb]{0.48,0.87,0.42}{0.56} & \colorbox[rgb]{0.92,0.46,0.43}{0.81} & \colorbox[rgb]{0.88,0.31,0.28}{0.99} & \colorbox[rgb]{0.88,0.33,0.29}{0.94} & \colorbox[rgb]{0.51,0.82,0.42}{0.82}  & 0.76 \\
\small 3402 & \colorbox[rgb]{0.84,0.81,0.68}{0.99} & \colorbox[rgb]{0.79,0.84,0.66}{0.95} & \colorbox[rgb]{0.74,0.69,0.51}{0.92} & \colorbox[rgb]{0.58,1.0,0.58}{0.68} & \colorbox[rgb]{0.74,0.8,0.59}{0.92} & \colorbox[rgb]{0.56,0.9,0.51}{1.00} & \colorbox[rgb]{0.75,0.83,0.62}{0.94} & \colorbox[rgb]{0.86,0.83,0.71}{0.96} & \colorbox[rgb]{0.94,0.74,0.7}{0.76} & \colorbox[rgb]{0.86,0.87,0.75}{0.97} & \colorbox[rgb]{0.65,0.97,0.63}{0.89} & \colorbox[rgb]{0.92,0.97,0.89}{0.99} & \colorbox[rgb]{0.73,0.85,0.62}{0.82} & \colorbox[rgb]{0.96,0.94,0.9}{0.46} & \colorbox[rgb]{0.96,0.96,0.92}{1.00} & \colorbox[rgb]{0.81,0.79,0.64}{0.95} & \colorbox[rgb]{0.85,0.99,0.84}{0.80}  & 0.88 \\
\small 4752 & \colorbox[rgb]{0.5,0.84,0.42}{0.97} & \colorbox[rgb]{0.48,0.92,0.44}{0.62} & \colorbox[rgb]{0.92,0.35,0.33}{0.39} & \colorbox[rgb]{0.73,0.8,0.58}{1.00} & \colorbox[rgb]{0.91,0.64,0.58}{0.86} & \colorbox[rgb]{0.69,0.57,0.4}{0.67} & \colorbox[rgb]{0.7,0.71,0.5}{0.73} & \colorbox[rgb]{0.63,0.79,0.5}{0.73} & \colorbox[rgb]{0.88,0.56,0.49}{0.88} & \colorbox[rgb]{0.65,0.93,0.61}{0.86} & \colorbox[rgb]{0.33,0.92,0.3}{1.00} & \colorbox[rgb]{0.84,0.97,0.82}{0.99} & \colorbox[rgb]{0.23,0.91,0.2}{0.98} & \colorbox[rgb]{0.33,0.96,0.31}{0.93} & \colorbox[rgb]{0.82,0.79,0.65}{0.92} & \colorbox[rgb]{0.71,0.75,0.53}{0.91} & \colorbox[rgb]{0.91,0.64,0.58}{0.82}  & 0.84 \\
\small 6188 & \colorbox[rgb]{0.88,0.79,0.69}{1.00} & \colorbox[rgb]{0.72,0.92,0.66}{0.94} & \colorbox[rgb]{0.78,0.68,0.53}{0.87} & \colorbox[rgb]{0.67,0.99,0.66}{0.93} & \colorbox[rgb]{0.64,0.89,0.57}{0.90} & \colorbox[rgb]{0.75,0.86,0.65}{0.88} & \colorbox[rgb]{0.64,0.87,0.56}{0.83} & \colorbox[rgb]{0.7,0.92,0.65}{0.90} & \colorbox[rgb]{0.97,0.7,0.68}{0.81} & \colorbox[rgb]{0.86,0.94,0.81}{0.90} & \colorbox[rgb]{0.82,0.79,0.65}{0.94} & \colorbox[rgb]{0.86,0.97,0.84}{0.99} & \colorbox[rgb]{0.89,0.73,0.65}{0.95} & \colorbox[rgb]{0.9,0.99,0.89}{0.58} & \colorbox[rgb]{0.98,0.98,0.96}{0.99} & \colorbox[rgb]{0.92,0.63,0.58}{0.80} & \colorbox[rgb]{0.95,0.86,0.82}{0.96}  & 0.89 \\
\small 6216 & \colorbox[rgb]{0.83,0.78,0.65}{0.98} & \colorbox[rgb]{0.55,0.94,0.52}{0.81} & \colorbox[rgb]{0.79,0.35,0.28}{0.86} & \colorbox[rgb]{0.31,1.0,0.31}{0.50} & \colorbox[rgb]{0.87,0.8,0.7}{0.94} & \colorbox[rgb]{0.65,0.84,0.55}{0.96} & \colorbox[rgb]{0.91,0.71,0.65}{0.92} & \colorbox[rgb]{0.79,0.86,0.68}{0.94} & \colorbox[rgb]{0.92,0.73,0.67}{0.77} & \colorbox[rgb]{0.85,0.94,0.8}{0.99} & \colorbox[rgb]{0.68,0.82,0.56}{0.83} & \colorbox[rgb]{0.97,0.93,0.9}{0.99} & \colorbox[rgb]{0.71,0.8,0.57}{0.93} & \colorbox[rgb]{1.0,0.66,0.66}{0.31} & \colorbox[rgb]{0.97,0.96,0.93}{1.00} & \colorbox[rgb]{0.89,0.71,0.63}{0.88} & \colorbox[rgb]{0.9,0.97,0.87}{0.99}  & 0.86 \\
\small 6619 & \colorbox[rgb]{0.77,0.75,0.58}{0.91} & \colorbox[rgb]{0.76,0.82,0.62}{0.80} & \colorbox[rgb]{0.47,0.79,0.37}{0.55} & \colorbox[rgb]{0.7,0.98,0.69}{0.92} & \colorbox[rgb]{0.9,0.75,0.67}{0.99} & \colorbox[rgb]{0.42,0.9,0.38}{0.73} & \colorbox[rgb]{0.84,0.61,0.51}{0.80} & \colorbox[rgb]{0.47,0.9,0.43}{0.58} & \colorbox[rgb]{0.94,0.37,0.35}{0.99} & \colorbox[rgb]{0.61,0.78,0.48}{0.87} & \colorbox[rgb]{0.89,0.74,0.66}{0.63} & \colorbox[rgb]{0.95,0.95,0.9}{1.00} & \colorbox[rgb]{0.86,0.54,0.47}{0.77} & \colorbox[rgb]{0.97,0.77,0.75}{0.58} & \colorbox[rgb]{0.76,0.98,0.75}{0.13} & \colorbox[rgb]{0.97,0.42,0.41}{0.77} & \colorbox[rgb]{0.8,0.91,0.73}{0.91}  & 0.76 \\
\small 6884 & \colorbox[rgb]{0.76,0.74,0.56}{0.94} & \colorbox[rgb]{0.45,0.94,0.43}{0.62} & \colorbox[rgb]{0.76,0.61,0.47}{0.93} & \colorbox[rgb]{0.62,0.99,0.62}{1.00} & \colorbox[rgb]{0.48,0.87,0.42}{0.80} & \colorbox[rgb]{0.71,0.72,0.51}{0.68} & \colorbox[rgb]{0.59,0.81,0.48}{0.68} & \colorbox[rgb]{0.58,0.81,0.47}{0.71} & \colorbox[rgb]{0.88,0.73,0.64}{0.94} & \colorbox[rgb]{0.75,0.79,0.59}{0.96} & \colorbox[rgb]{0.47,0.88,0.42}{0.64} & \colorbox[rgb]{0.83,0.96,0.8}{0.98} & \colorbox[rgb]{0.6,0.83,0.5}{0.86} & \colorbox[rgb]{0.72,0.98,0.71}{0.58} & \colorbox[rgb]{0.99,0.84,0.83}{0.96} & \colorbox[rgb]{0.82,0.73,0.6}{0.92} & \colorbox[rgb]{0.95,0.78,0.74}{0.74}  & 0.82 \\
\small 7502 & \colorbox[rgb]{0.78,0.86,0.67}{0.96} & \colorbox[rgb]{0.65,0.98,0.64}{0.88} & \colorbox[rgb]{0.75,0.71,0.53}{0.92} & \colorbox[rgb]{0.64,1.0,0.64}{0.89} & \colorbox[rgb]{0.86,0.78,0.67}{0.96} & \colorbox[rgb]{0.75,0.78,0.59}{0.80} & \colorbox[rgb]{0.82,0.78,0.64}{0.93} & \colorbox[rgb]{0.78,0.92,0.72}{0.95} & \colorbox[rgb]{0.91,0.76,0.69}{0.90} & \colorbox[rgb]{0.88,0.96,0.84}{0.99} & \colorbox[rgb]{0.7,0.96,0.67}{0.93} & \colorbox[rgb]{0.89,0.97,0.86}{1.00} & \colorbox[rgb]{0.76,0.85,0.65}{0.71} & \colorbox[rgb]{0.91,0.99,0.9}{0.39} & \colorbox[rgb]{0.97,0.97,0.94}{1.00} & \colorbox[rgb]{0.86,0.78,0.67}{0.97} & \colorbox[rgb]{0.93,0.94,0.87}{0.98}  & 0.89 \\
\small 8387 & \colorbox[rgb]{0.73,0.75,0.55}{0.85} & \colorbox[rgb]{0.78,0.7,0.55}{1.00} & \colorbox[rgb]{0.65,0.85,0.55}{0.63} & \colorbox[rgb]{0.73,0.89,0.65}{0.98} & \colorbox[rgb]{0.84,0.63,0.53}{0.79} & \colorbox[rgb]{0.93,0.39,0.36}{0.89} & \colorbox[rgb]{0.81,0.63,0.51}{0.76} & \colorbox[rgb]{0.74,0.6,0.45}{0.71} & \colorbox[rgb]{0.8,0.62,0.5}{0.99} & \colorbox[rgb]{0.47,0.86,0.41}{0.91} & \colorbox[rgb]{0.78,0.73,0.57}{0.88} & \colorbox[rgb]{0.94,0.68,0.64}{0.42} & \colorbox[rgb]{0.63,0.87,0.55}{0.65} & \colorbox[rgb]{0.75,0.97,0.73}{0.92} & \colorbox[rgb]{0.82,0.77,0.63}{0.68} & \colorbox[rgb]{0.97,0.66,0.64}{1.00} & \colorbox[rgb]{0.89,0.77,0.69}{0.97}  & 0.83 \\
\small 10096 & \colorbox[rgb]{0.73,0.7,0.51}{0.65} & \colorbox[rgb]{0.62,0.73,0.45}{0.73} & \colorbox[rgb]{0.63,0.66,0.42}{0.90} & \colorbox[rgb]{0.85,0.59,0.5}{0.96} & \colorbox[rgb]{0.85,0.55,0.47}{0.81} & \colorbox[rgb]{0.86,0.39,0.34}{1.00} & \colorbox[rgb]{0.8,0.66,0.53}{0.85} & \colorbox[rgb]{0.74,0.51,0.38}{0.51} & \colorbox[rgb]{0.72,0.93,0.67}{0.78} & \colorbox[rgb]{0.7,0.73,0.51}{0.60} & \colorbox[rgb]{0.76,0.75,0.57}{0.53} & \colorbox[rgb]{0.7,0.73,0.51}{0.98} & \colorbox[rgb]{0.64,0.94,0.6}{0.95} & \colorbox[rgb]{0.99,0.87,0.86}{0.71} & \colorbox[rgb]{1.0,0.37,0.37}{0.90} & \colorbox[rgb]{0.7,0.73,0.51}{0.83} & \colorbox[rgb]{0.9,0.59,0.53}{0.80}  & 0.79 \\
\small 10454 & \colorbox[rgb]{0.8,0.79,0.63}{0.98} & \colorbox[rgb]{0.47,0.96,0.45}{0.58} & \colorbox[rgb]{0.74,0.66,0.49}{0.89} & \colorbox[rgb]{0.61,0.99,0.6}{0.89} & \colorbox[rgb]{0.8,0.82,0.66}{0.99} & \colorbox[rgb]{0.56,0.81,0.45}{0.85} & \colorbox[rgb]{0.91,0.67,0.61}{0.90} & \colorbox[rgb]{0.64,0.95,0.61}{0.86} & \colorbox[rgb]{0.97,0.53,0.52}{0.93} & \colorbox[rgb]{0.75,0.95,0.71}{0.98} & \colorbox[rgb]{0.51,0.97,0.5}{0.77} & \colorbox[rgb]{0.92,0.96,0.88}{1.00} & \colorbox[rgb]{0.64,0.89,0.57}{0.81} & \colorbox[rgb]{0.99,0.92,0.91}{0.42} & \colorbox[rgb]{0.97,0.96,0.93}{1.00} & \colorbox[rgb]{0.84,0.68,0.57}{0.98} & \colorbox[rgb]{0.83,0.95,0.79}{0.95}  & 0.87 \\
\small 10605 & \colorbox[rgb]{0.54,0.8,0.44}{0.88} & \colorbox[rgb]{0.47,0.87,0.41}{1.00} & \colorbox[rgb]{0.73,0.53,0.39}{0.89} & \colorbox[rgb]{0.58,0.98,0.57}{0.83} & \colorbox[rgb]{0.42,0.88,0.36}{0.73} & \colorbox[rgb]{0.86,0.44,0.37}{0.47} & \colorbox[rgb]{0.45,0.93,0.42}{0.65} & \colorbox[rgb]{0.38,0.96,0.37}{0.85} & \colorbox[rgb]{0.98,0.68,0.67}{0.76} & \colorbox[rgb]{0.62,0.8,0.5}{0.72} & \colorbox[rgb]{0.46,0.89,0.41}{0.97} & \colorbox[rgb]{0.86,0.96,0.82}{0.98} & \colorbox[rgb]{0.56,0.83,0.47}{0.72} & \colorbox[rgb]{0.83,0.97,0.8}{0.99} & \colorbox[rgb]{0.97,0.64,0.62}{0.80} & \colorbox[rgb]{0.83,0.58,0.48}{0.96} & \colorbox[rgb]{0.84,0.9,0.76}{0.52}  & 0.81 \\
\small 11712 & \colorbox[rgb]{0.88,0.89,0.78}{0.95} & \colorbox[rgb]{0.86,0.77,0.66}{0.98} & \colorbox[rgb]{0.73,0.72,0.53}{0.86} & \colorbox[rgb]{0.94,0.99,0.93}{0.95} & \colorbox[rgb]{0.78,0.91,0.71}{0.80} & \colorbox[rgb]{0.66,0.9,0.6}{0.90} & \colorbox[rgb]{0.8,0.75,0.6}{0.89} & \colorbox[rgb]{0.71,0.84,0.6}{0.86} & \colorbox[rgb]{0.93,0.85,0.79}{0.92} & \colorbox[rgb]{0.81,0.97,0.78}{0.94} & \colorbox[rgb]{0.63,0.91,0.58}{0.87} & \colorbox[rgb]{0.97,0.92,0.89}{1.00} & \colorbox[rgb]{0.53,0.86,0.46}{0.87} & \colorbox[rgb]{0.99,0.99,0.98}{0.70} & \colorbox[rgb]{0.83,0.88,0.73}{0.86} & \colorbox[rgb]{0.87,0.86,0.75}{0.80} & \colorbox[rgb]{0.89,0.91,0.81}{0.75}  & 0.88 \\
\small 12703 & \colorbox[rgb]{0.83,0.83,0.69}{0.94} & \colorbox[rgb]{0.87,0.85,0.74}{0.96} & \colorbox[rgb]{0.74,0.52,0.39}{0.91} & \colorbox[rgb]{0.38,0.99,0.38}{0.52} & \colorbox[rgb]{0.76,0.87,0.66}{0.98} & \colorbox[rgb]{0.61,0.92,0.56}{0.77} & \colorbox[rgb]{0.71,0.87,0.62}{0.91} & \colorbox[rgb]{0.74,0.87,0.64}{0.91} & \colorbox[rgb]{0.94,0.64,0.6}{0.75} & \colorbox[rgb]{0.87,0.85,0.74}{0.99} & \colorbox[rgb]{0.82,0.9,0.74}{0.97} & \colorbox[rgb]{0.96,0.98,0.94}{0.98} & \colorbox[rgb]{0.67,0.86,0.58}{0.96} & \colorbox[rgb]{0.98,0.61,0.6}{0.44} & \colorbox[rgb]{0.97,0.98,0.95}{1.00} & \colorbox[rgb]{0.9,0.69,0.62}{0.74} & \colorbox[rgb]{0.89,0.94,0.84}{0.97}  & 0.86 \\
\small 14049 & \colorbox[rgb]{0.65,0.78,0.51}{0.98} & \colorbox[rgb]{0.44,0.9,0.39}{0.59} & \colorbox[rgb]{0.68,0.72,0.49}{0.83} & \colorbox[rgb]{0.59,0.98,0.58}{0.99} & \colorbox[rgb]{0.65,0.87,0.57}{0.87} & \colorbox[rgb]{0.73,0.6,0.44}{0.51} & \colorbox[rgb]{0.24,0.94,0.22}{0.95} & \colorbox[rgb]{0.84,0.53,0.45}{0.65} & \colorbox[rgb]{0.88,0.68,0.6}{0.75} & \colorbox[rgb]{0.71,0.79,0.56}{0.89} & \colorbox[rgb]{0.47,0.88,0.42}{0.66} & \colorbox[rgb]{0.88,0.84,0.74}{0.99} & \colorbox[rgb]{0.65,0.72,0.47}{0.67} & \colorbox[rgb]{0.98,0.56,0.55}{0.84} & \colorbox[rgb]{0.93,0.62,0.58}{0.69} & \colorbox[rgb]{0.92,0.45,0.42}{1.00} & \colorbox[rgb]{0.73,0.87,0.64}{0.95}  & 0.81 \\
\small 14185 & \colorbox[rgb]{0.7,0.78,0.55}{0.99} & \colorbox[rgb]{0.8,0.71,0.57}{0.95} & \colorbox[rgb]{0.76,0.66,0.5}{0.96} & \colorbox[rgb]{0.82,0.92,0.75}{0.99} & \colorbox[rgb]{0.81,0.79,0.64}{0.62} & \colorbox[rgb]{0.57,0.81,0.46}{0.78} & \colorbox[rgb]{0.67,0.77,0.52}{0.88} & \colorbox[rgb]{0.87,0.63,0.55}{0.79} & \colorbox[rgb]{0.96,0.62,0.6}{0.77} & \colorbox[rgb]{0.69,0.88,0.61}{0.98} & \colorbox[rgb]{0.75,0.91,0.68}{0.95} & \colorbox[rgb]{0.81,0.96,0.78}{1.00} & \colorbox[rgb]{0.69,0.8,0.55}{0.86} & \colorbox[rgb]{0.83,0.94,0.78}{0.91} & \colorbox[rgb]{0.97,0.81,0.78}{0.96} & \colorbox[rgb]{0.93,0.72,0.67}{0.76} & \colorbox[rgb]{0.79,0.96,0.76}{0.59}  & 0.87 \\
\small 14351 & \colorbox[rgb]{0.86,0.83,0.71}{0.99} & \colorbox[rgb]{0.61,0.97,0.59}{0.83} & \colorbox[rgb]{0.75,0.75,0.56}{0.90} & \colorbox[rgb]{0.63,0.99,0.62}{0.86} & \colorbox[rgb]{0.68,0.9,0.61}{0.93} & \colorbox[rgb]{0.76,0.81,0.62}{0.75} & \colorbox[rgb]{0.9,0.74,0.67}{0.92} & \colorbox[rgb]{0.81,0.93,0.75}{0.97} & \colorbox[rgb]{0.92,0.76,0.7}{0.41} & \colorbox[rgb]{0.85,0.97,0.82}{0.99} & \colorbox[rgb]{0.71,0.98,0.7}{0.92} & \colorbox[rgb]{0.95,0.97,0.92}{1.00} & \colorbox[rgb]{0.64,0.82,0.53}{0.92} & \colorbox[rgb]{0.97,0.97,0.94}{0.45} & \colorbox[rgb]{0.94,0.99,0.93}{1.00} & \colorbox[rgb]{0.89,0.74,0.66}{0.93} & \colorbox[rgb]{0.86,0.99,0.85}{0.98}  & 0.87 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

\makecell{\textbf{1312}} & \cellbar{0.14}{0.96}{0.60}{0.26}{0.40} & \cellbar{0.21}{0.96}{0.65}{0.14}{0.35} & \cellbar{0.77}{0.99}{0.08}{0.15}{0.92} & \cellbar{0.00}{0.41}{0.29}{0.71}{0.71} & \cellbar{0.16}{0.78}{0.38}{0.47}{0.62} & \cellbar{0.09}{0.94}{0.64}{0.27}{0.36} & \cellbar{0.23}{0.91}{0.58}{0.19}{0.42} & \cellbar{0.26}{0.65}{0.68}{0.06}{0.32} & \cellbar{0.55}{0.66}{0.41}{0.04}{0.59} & \cellbar{0.15}{0.88}{0.52}{0.33}{0.48} & \cellbar{0.07}{0.47}{0.18}{0.75}{0.82} & \cellbar{0.71}{0.93}{0.29}{0.00}{0.71} & 0.79 \\
\makecell{\textbf{1975}} & \cellbar{0.11}{0.88}{0.66}{0.23}{0.34} & \cellbar{0.18}{0.81}{0.42}{0.41}{0.58} & \cellbar{0.25}{0.84}{0.41}{0.35}{0.59} & \cellbar{0.05}{0.96}{0.71}{0.24}{0.29} & \cellbar{0.02}{0.65}{0.35}{0.63}{0.65} & \cellbar{0.47}{0.68}{0.39}{0.15}{0.61} & \cellbar{0.12}{0.78}{0.50}{0.39}{0.50} & \cellbar{0.66}{0.92}{0.23}{0.11}{0.77} & \cellbar{0.18}{0.66}{0.48}{0.35}{0.52} & \cellbar{0.12}{0.68}{0.70}{0.18}{0.30} & \cellbar{0.21}{0.74}{0.69}{0.10}{0.31} & \cellbar{0.25}{0.99}{0.64}{0.11}{0.36} & 0.80 \\
\makecell{\textbf{3183}} & \cellbar{0.19}{0.95}{0.22}{0.59}{0.78} & \cellbar{0.58}{0.67}{0.16}{0.26}{0.84} & \cellbar{0.68}{0.97}{0.18}{0.14}{0.82} & \cellbar{0.16}{0.80}{0.35}{0.50}{0.65} & \cellbar{0.20}{0.97}{0.20}{0.60}{0.80} & \cellbar{0.22}{0.75}{0.36}{0.43}{0.64} & \cellbar{0.40}{0.74}{0.24}{0.37}{0.76} & \cellbar{0.33}{0.88}{0.35}{0.33}{0.65} & \cellbar{0.76}{0.16}{0.16}{0.08}{0.84} & \cellbar{0.46}{0.53}{0.48}{0.07}{0.52} & \cellbar{0.13}{0.56}{0.36}{0.51}{0.64} & \cellbar{0.67}{0.94}{0.21}{0.12}{0.79} & 0.74 \\
\makecell{\textbf{4752}} & \cellbar{0.16}{0.97}{0.35}{0.50}{0.65} & \cellbar{0.08}{0.62}{0.41}{0.51}{0.59} & \cellbar{0.64}{0.39}{0.28}{0.08}{0.72} & \cellbar{0.20}{1.00}{0.53}{0.27}{0.47} & \cellbar{0.43}{0.67}{0.27}{0.31}{0.73} & \cellbar{0.29}{0.73}{0.42}{0.30}{0.58} & \cellbar{0.21}{0.73}{0.43}{0.37}{0.57} & \cellbar{0.44}{0.88}{0.45}{0.12}{0.55} & \cellbar{0.07}{0.86}{0.58}{0.35}{0.42} & \cellbar{0.08}{1.00}{0.25}{0.67}{0.75} & \cellbar{0.09}{0.98}{0.14}{0.77}{0.86} & \cellbar{0.25}{0.91}{0.47}{0.29}{0.53} & 0.81 \\
\makecell{\textbf{6216}} & \cellbar{0.22}{0.98}{0.61}{0.17}{0.39} & \cellbar{0.06}{0.81}{0.50}{0.45}{0.50} & \cellbar{0.64}{0.86}{0.15}{0.21}{0.85} & \cellbar{0.00}{0.50}{0.32}{0.68}{0.68} & \cellbar{0.16}{0.96}{0.50}{0.35}{0.50} & \cellbar{0.29}{0.92}{0.62}{0.09}{0.38} & \cellbar{0.14}{0.94}{0.65}{0.21}{0.35} & \cellbar{0.27}{0.77}{0.65}{0.08}{0.35} & \cellbar{0.06}{0.99}{0.79}{0.15}{0.21} & \cellbar{0.18}{0.83}{0.50}{0.32}{0.50} & \cellbar{0.20}{0.93}{0.51}{0.29}{0.49} & \cellbar{0.29}{0.88}{0.60}{0.11}{0.40} & 0.87 \\
\makecell{\textbf{6619}} & \cellbar{0.25}{0.91}{0.52}{0.23}{0.48} & \cellbar{0.18}{0.80}{0.58}{0.24}{0.42} & \cellbar{0.21}{0.55}{0.27}{0.52}{0.73} & \cellbar{0.02}{0.92}{0.68}{0.30}{0.32} & \cellbar{0.10}{0.73}{0.33}{0.57}{0.67} & \cellbar{0.39}{0.80}{0.46}{0.16}{0.54} & \cellbar{0.10}{0.58}{0.38}{0.52}{0.62} & \cellbar{0.62}{0.99}{0.32}{0.06}{0.68} & \cellbar{0.22}{0.87}{0.40}{0.39}{0.60} & \cellbar{0.26}{0.63}{0.63}{0.11}{0.37} & \cellbar{0.46}{0.77}{0.41}{0.14}{0.59} & \cellbar{0.57}{0.77}{0.40}{0.03}{0.60} & 0.78 \\
\makecell{\textbf{8387}} & \cellbar{0.25}{0.85}{0.49}{0.27}{0.51} & \cellbar{0.30}{1.00}{0.49}{0.22}{0.51} & \cellbar{0.15}{0.63}{0.50}{0.35}{0.50} & \cellbar{0.11}{0.98}{0.62}{0.27}{0.38} & \cellbar{0.60}{0.89}{0.33}{0.07}{0.67} & \cellbar{0.37}{0.76}{0.45}{0.19}{0.55} & \cellbar{0.40}{0.71}{0.35}{0.26}{0.65} & \cellbar{0.38}{0.99}{0.43}{0.20}{0.57} & \cellbar{0.14}{0.91}{0.34}{0.52}{0.66} & \cellbar{0.27}{0.88}{0.51}{0.22}{0.49} & \cellbar{0.13}{0.65}{0.50}{0.37}{0.50} & \cellbar{0.34}{1.00}{0.63}{0.03}{0.37} & 0.85 \\
\makecell{\textbf{10096}} & \cellbar{0.30}{0.65}{0.44}{0.27}{0.56} & \cellbar{0.27}{0.73}{0.36}{0.38}{0.64} & \cellbar{0.34}{0.90}{0.30}{0.37}{0.70} & \cellbar{0.41}{0.96}{0.45}{0.15}{0.55} & \cellbar{0.60}{1.00}{0.26}{0.14}{0.74} & \cellbar{0.34}{0.85}{0.47}{0.20}{0.53} & \cellbar{0.49}{0.51}{0.26}{0.26}{0.74} & \cellbar{0.07}{0.78}{0.65}{0.28}{0.35} & \cellbar{0.27}{0.60}{0.44}{0.30}{0.56} & \cellbar{0.25}{0.53}{0.51}{0.24}{0.49} & \cellbar{0.06}{0.95}{0.58}{0.36}{0.42} & \cellbar{0.27}{0.83}{0.44}{0.30}{0.56} & 0.77 \\
\makecell{\textbf{10605}} & \cellbar{0.20}{0.88}{0.35}{0.46}{0.65} & \cellbar{0.13}{1.00}{0.35}{0.52}{0.65} & \cellbar{0.47}{0.89}{0.27}{0.27}{0.73} & \cellbar{0.02}{0.83}{0.56}{0.42}{0.44} & \cellbar{0.56}{0.47}{0.30}{0.14}{0.70} & \cellbar{0.07}{0.65}{0.39}{0.54}{0.61} & \cellbar{0.04}{0.85}{0.35}{0.61}{0.65} & \cellbar{0.32}{0.76}{0.66}{0.02}{0.34} & \cellbar{0.20}{0.72}{0.43}{0.38}{0.57} & \cellbar{0.11}{0.97}{0.36}{0.53}{0.64} & \cellbar{0.17}{0.72}{0.40}{0.44}{0.60} & \cellbar{0.42}{0.96}{0.42}{0.17}{0.58} & 0.81 \\
\makecell{\textbf{14049}} & \cellbar{0.22}{0.98}{0.44}{0.35}{0.56} & \cellbar{0.10}{0.59}{0.34}{0.56}{0.66} & \cellbar{0.28}{0.83}{0.41}{0.32}{0.59} & \cellbar{0.02}{0.99}{0.57}{0.41}{0.43} & \cellbar{0.40}{0.51}{0.34}{0.27}{0.66} & \cellbar{0.06}{0.95}{0.18}{0.76}{0.82} & \cellbar{0.47}{0.65}{0.38}{0.16}{0.62} & \cellbar{0.32}{0.75}{0.56}{0.12}{0.44} & \cellbar{0.21}{0.89}{0.50}{0.29}{0.50} & \cellbar{0.12}{0.66}{0.36}{0.52}{0.64} & \cellbar{0.28}{0.67}{0.38}{0.35}{0.62} & \cellbar{0.54}{1.00}{0.38}{0.08}{0.62} & 0.79 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\caption{Score changes in other value dimensions when steering a single dimension via prompts. We separately present the changes in scores for values that are expected to be influenced according to the causal graph and for those that are unexpectedly affected. }
\label{table: scorechange}
\begin{center}
\begin{tabular}{c@{\hspace{2pt}}|c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}|c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}}
\toprule
 & \multicolumn{4}{c|}{\bf \small Gemma-2B-IT} & \multicolumn{4}{c}{\bf \small Llama3-8B-IT}\\
 \hline
Value Dimensions & \multicolumn{2}{c|}{\bf \tiny Our causal graph} & \multicolumn{2}{c|}{\bf \tiny Human annotated graph} & \multicolumn{2}{c|}{\bf \tiny Our causal graph} & \multicolumn{2}{c}{\bf \tiny Human annotated graph}  \\
Score Change & \multicolumn{1}{c}{\bf \tiny Expected} & \multicolumn{1}{c|}{\bf \tiny Unexpected} & \multicolumn{1}{c}{\bf \tiny Expected} & \multicolumn{1}{c|}{\bf \tiny Unexpected} & \multicolumn{1}{c}{\bf \tiny Expected} & \multicolumn{1}{c|}{\bf \tiny Unexpected} & \multicolumn{1}{c}{\bf \tiny Expected} & \multicolumn{1}{c}{\bf \tiny Unexpected}\\
\hline
\small Affiliation & 0.19 & 0.08 & 0.13 & 0.16 & 0.18 & 0.08 & 0.14 & 0.17  \\
\small Assertiveness & 0.18 & 0.06 & nan & 0.14 & 0.19 & 0.08 & nan & 0.16  \\
\small Behavioral Inhibition System & nan & 0.15 & nan & 0.15 & nan & 0.15 & nan & 0.15  \\
\small Breadth of Interest & 0.2 & 0.08 & nan & 0.15 & nan & 0.16 & nan & 0.16  \\
\small Complexity & nan & nan & nan & nan & 0.33 & 0.27 & nan & 0.28  \\
\small Dependence & 0.17 & 0.12 & 0.15 & 0.15 & nan & 0.2 & 0.19 & 0.23  \\
\small Depth & 0.21 & 0.07 & nan & 0.16 & 0.2 & 0.15 & nan & 0.15  \\
\small Emotional Expression & nan & nan & nan & nan & 0.08 & 0.14 & nan & 0.13  \\
\small Emotional Processing & 0.22 & 0.1 & 0.14 & 0.21 & nan & nan & nan & nan  \\
\small Empathy & 0.19 & 0.08 & 0.14 & 0.16 & 0.25 & 0.14 & 0.15 & 0.16  \\
\small Extraversion & 0.2 & 0.08 & 0.13 & 0.17 & 0.18 & 0.08 & 0.14 & 0.16  \\
\small Imagination & 0.17 & 0.09 & nan & 0.14 & 0.26 & 0.21 & nan & 0.22  \\
\small Nurturance & nan & 0.14 & 0.12 & 0.15 & 0.21 & 0.13 & 0.13 & 0.16  \\
\small Perspective Taking & nan & nan & nan & nan & nan & 0.16 & 0.16 & 0.16  \\
\small Poise & 0.18 & 0.08 & nan & 0.14 & 0.19 & 0.08 & nan & 0.16  \\
\small Positive Expressivity & 0.18 & 0.07 & 0.13 & 0.15 & 0.19 & 0.13 & 0.13 & 0.16  \\
\small Preference for Order and Structure & 0.19 & 0.08 & nan & 0.14 & 0.21 & 0.15 & nan & 0.16  \\
\small Privacy & nan & nan & nan & nan & nan & nan & nan & nan  \\
\small Psychosocial flourishing & 0.18 & 0.08 & nan & 0.14 & 0.06 & 0.16 & nan & 0.16  \\
\small Reflection & 0.16 & 0.09 & 0.13 & 0.14 & 0.19 & 0.16 & 0.16 & 0.17  \\
\small Satisfaction with life & 0.17 & 0.09 & nan & 0.14 & 0.2 & 0.13 & nan & 0.15  \\
\small Sociability & 0.17 & 0.1 & 0.14 & 0.14 & 0.09 & 0.16 & 0.14 & 0.16  \\
\small Social & 0.19 & 0.06 & 0.13 & 0.16 & 0.2 & 0.15 & 0.15 & 0.16  \\
\small Social Confidence & 0.19 & 0.08 & nan & 0.14 & 0.18 & 0.08 & nan & 0.16  \\
\small Social Withdrawal & 0.18 & 0.08 & nan & 0.14 & 0.19 & 0.15 & nan & 0.16  \\
\small Sympathy & 0.17 & 0.07 & 0.13 & 0.15 & 0.19 & 0.15 & 0.16 & 0.18  \\
\small Tenderness & 0.17 & 0.09 & 0.14 & 0.14 & 0.23 & 0.15 & 0.16 & 0.18  \\
\small Theoretical & 0.18 & 0.08 & 0.14 & 0.15 & 0.2 & 0.14 & 0.15 & 0.16  \\
\small Understanding & 0.17 & 0.09 & 0.14 & 0.14 & 0.19 & 0.08 & 0.15 & 0.18  \\
\small Warmth & nan & nan & nan & nan & nan & nan & nan & nan  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{CustomBlue}{HTML}{42A5F5}
\definecolor{CustomYellow}{HTML}{FFCA28}
\definecolor{DarkCBlue}{HTML}{9F9FFF}
\definecolor{DarkCRed}{HTML}{FF7F7F}
% \definecolor{DarkCBlue}{HTML}{6b6bdf}
% \definecolor{DarkCRed}{HTML}{e04646}


\newcommand{\cellbar}[5]{%
    \raisebox{\height}{%
        \begin{tikzpicture}[baseline=(current bounding box.center)]
            \draw[draw=black] (0,0) rectangle (1cm,0.4cm);
            \path[fill=CustomBlue, opacity=#5] (0,0) rectangle (#1cm,0.4cm);
            \path[fill=white] (#1cm,0) rectangle ({#1cm + #3cm},0.4cm);
            \path[fill=CustomYellow, opacity=#5] ({#1cm + #3cm},0) rectangle (1cm,0.4cm);
            \node[anchor=center, font=\scriptsize] at (0.5cm,0.2cm) {#2};
        \end{tikzpicture}%
    }%
}

\begin{table*}[ht]
\centering
\caption{Value steering using SAE features for the {Gemma-2B-IT} model. For each pair of steering feature and value dimension, the cell shows the stimulation ratio in blue, the suppression ratio in yellow, and the maintenance ratio in blank, which are estimated from the training data. The numbers in the cell represent the distance between the actual ratios in the testing data and expected ratios.}

\label{table: sae-steering-gemma}
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} *{12}{>{\centering\arraybackslash}m{1cm}}>{\centering\arraybackslash}m{1cm}}
\toprule
\rotatebox{90}{\textbf{Value}} & \rotatebox{90}{\textbf{Achievement}} & \rotatebox{90}{\textbf{Aesthetic}} & \rotatebox{90}{\textbf{Anxiety Disorder}} & \rotatebox{90}{\textbf{Breadth of Interest}} & \rotatebox{90}{\textbf{Empathy}} & \rotatebox{90}{\textbf{Organization}} & \rotatebox{90}{\textbf{Political}} & \rotatebox{90}{\textbf{Positive coping}} & \rotatebox{90}{\textbf{Religious}} & \rotatebox{90}{\textbf{Resilience}} & \rotatebox{90}{\textbf{Social Complexity}} & \rotatebox{90}{\textbf{Uncertainty Avoidance}} & \textbf{AVG} \\
\midrule
\textbf{428} & \cellbar{0.19}{0.90}{0.58}{0.23}{0.42} & \cellbar{0.15}{0.96}{0.62}{0.23}{0.38} & \cellbar{0.46}{0.90}{0.36}{0.19}{0.64} & \cellbar{0.03}{0.94}{0.65}{0.32}{0.35} & \cellbar{0.23}{0.60}{0.49}{0.29}{0.51} & \cellbar{0.57}{0.57}{0.36}{0.07}{0.64} & \cellbar{0.49}{0.65}{0.40}{0.12}{0.60} & \cellbar{0.30}{0.98}{0.62}{0.08}{0.38} & \cellbar{0.20}{0.92}{0.58}{0.22}{0.42} & \cellbar{0.22}{0.97}{0.59}{0.19}{0.41} & \cellbar{0.17}{0.87}{0.52}{0.31}{0.48} & \cellbar{0.45}{0.89}{0.49}{0.07}{0.51} & 0.85 \\
\textbf{1312} & \cellbar{0.14}{0.96}{0.60}{0.26}{0.40} & \cellbar{0.21}{0.96}{0.65}{0.14}{0.35} & \cellbar{0.77}{0.99}{0.08}{0.15}{0.92} & \cellbar{0.00}{0.41}{0.29}{0.71}{0.71} & \cellbar{0.16}{0.78}{0.38}{0.47}{0.62} & \cellbar{0.09}{0.94}{0.64}{0.27}{0.36} & \cellbar{0.23}{0.91}{0.58}{0.19}{0.42} & \cellbar{0.26}{0.65}{0.68}{0.06}{0.32} & \cellbar{0.55}{0.66}{0.41}{0.04}{0.59} & \cellbar{0.15}{0.88}{0.52}{0.33}{0.48} & \cellbar{0.07}{0.47}{0.18}{0.75}{0.82} & \cellbar{0.71}{0.93}{0.29}{0.00}{0.71} & 0.79 \\
\textbf{1975} & \cellbar{0.11}{0.88}{0.66}{0.23}{0.34} & \cellbar{0.18}{0.81}{0.42}{0.41}{0.58} & \cellbar{0.25}{0.84}{0.41}{0.35}{0.59} & \cellbar{0.05}{0.96}{0.71}{0.24}{0.29} & \cellbar{0.02}{0.65}{0.35}{0.63}{0.65} & \cellbar{0.47}{0.68}{0.39}{0.15}{0.61} & \cellbar{0.12}{0.78}{0.50}{0.39}{0.50} & \cellbar{0.66}{0.92}{0.23}{0.11}{0.77} & \cellbar{0.18}{0.66}{0.48}{0.35}{0.52} & \cellbar{0.12}{0.68}{0.70}{0.18}{0.30} & \cellbar{0.21}{0.74}{0.69}{0.10}{0.31} & \cellbar{0.25}{0.99}{0.64}{0.11}{0.36} & 0.80 \\
\textbf{3183} & \cellbar{0.19}{0.95}{0.22}{0.59}{0.78} & \cellbar{0.58}{0.67}{0.16}{0.26}{0.84} & \cellbar{0.68}{0.97}{0.18}{0.14}{0.82} & \cellbar{0.16}{0.80}{0.35}{0.50}{0.65} & \cellbar{0.20}{0.97}{0.20}{0.60}{0.80} & \cellbar{0.22}{0.75}{0.36}{0.43}{0.64} & \cellbar{0.40}{0.74}{0.24}{0.37}{0.76} & \cellbar{0.33}{0.88}{0.35}{0.33}{0.65} & \cellbar{0.76}{0.16}{0.16}{0.08}{0.84} & \cellbar{0.46}{0.53}{0.48}{0.07}{0.52} & \cellbar{0.13}{0.56}{0.36}{0.51}{0.64} & \cellbar{0.67}{0.94}{0.21}{0.12}{0.79} & 0.74 \\
\textbf{4752} & \cellbar{0.16}{0.97}{0.35}{0.50}{0.65} & \cellbar{0.08}{0.62}{0.41}{0.51}{0.59} & \cellbar{0.64}{0.39}{0.28}{0.08}{0.72} & \cellbar{0.20}{1.00}{0.53}{0.27}{0.47} & \cellbar{0.43}{0.67}{0.27}{0.31}{0.73} & \cellbar{0.29}{0.73}{0.42}{0.30}{0.58} & \cellbar{0.21}{0.73}{0.43}{0.37}{0.57} & \cellbar{0.44}{0.88}{0.45}{0.12}{0.55} & \cellbar{0.07}{0.86}{0.58}{0.35}{0.42} & \cellbar{0.08}{1.00}{0.25}{0.67}{0.75} & \cellbar{0.09}{0.98}{0.14}{0.77}{0.86} & \cellbar{0.25}{0.91}{0.47}{0.29}{0.53} & 0.81 \\
\textbf{6216} & \cellbar{0.22}{0.98}{0.61}{0.17}{0.39} & \cellbar{0.06}{0.81}{0.50}{0.45}{0.50} & \cellbar{0.64}{0.86}{0.15}{0.21}{0.85} & \cellbar{0.00}{0.50}{0.32}{0.68}{0.68} & \cellbar{0.16}{0.96}{0.50}{0.35}{0.50} & \cellbar{0.29}{0.92}{0.62}{0.09}{0.38} & \cellbar{0.14}{0.94}{0.65}{0.21}{0.35} & \cellbar{0.27}{0.77}{0.65}{0.08}{0.35} & \cellbar{0.06}{0.99}{0.79}{0.15}{0.21} & \cellbar{0.18}{0.83}{0.50}{0.32}{0.50} & \cellbar{0.20}{0.93}{0.51}{0.29}{0.49} & \cellbar{0.29}{0.88}{0.60}{0.11}{0.40} & 0.87 \\
\textbf{6619} & \cellbar{0.25}{0.91}{0.52}{0.23}{0.48} & \cellbar{0.18}{0.80}{0.58}{0.24}{0.42} & \cellbar{0.21}{0.55}{0.27}{0.52}{0.73} & \cellbar{0.02}{0.92}{0.68}{0.30}{0.32} & \cellbar{0.10}{0.73}{0.33}{0.57}{0.67} & \cellbar{0.39}{0.80}{0.46}{0.16}{0.54} & \cellbar{0.10}{0.58}{0.38}{0.52}{0.62} & \cellbar{0.62}{0.99}{0.32}{0.06}{0.68} & \cellbar{0.22}{0.87}{0.40}{0.39}{0.60} & \cellbar{0.26}{0.63}{0.63}{0.11}{0.37} & \cellbar{0.46}{0.77}{0.41}{0.14}{0.59} & \cellbar{0.57}{0.77}{0.40}{0.03}{0.60} & 0.78 \\
\textbf{8387} & \cellbar{0.25}{0.85}{0.49}{0.27}{0.51} & \cellbar{0.30}{1.00}{0.49}{0.22}{0.51} & \cellbar{0.15}{0.63}{0.50}{0.35}{0.50} & \cellbar{0.11}{0.98}{0.62}{0.27}{0.38} & \cellbar{0.60}{0.89}{0.33}{0.07}{0.67} & \cellbar{0.37}{0.76}{0.45}{0.19}{0.55} & \cellbar{0.40}{0.71}{0.35}{0.26}{0.65} & \cellbar{0.38}{0.99}{0.43}{0.20}{0.57} & \cellbar{0.14}{0.91}{0.34}{0.52}{0.66} & \cellbar{0.27}{0.88}{0.51}{0.22}{0.49} & \cellbar{0.13}{0.65}{0.50}{0.37}{0.50} & \cellbar{0.34}{1.00}{0.63}{0.03}{0.37} & 0.85 \\
\textbf{10096} & \cellbar{0.30}{0.65}{0.44}{0.27}{0.56} & \cellbar{0.27}{0.73}{0.36}{0.38}{0.64} & \cellbar{0.34}{0.90}{0.30}{0.37}{0.70} & \cellbar{0.41}{0.96}{0.45}{0.15}{0.55} & \cellbar{0.60}{1.00}{0.26}{0.14}{0.74} & \cellbar{0.34}{0.85}{0.47}{0.20}{0.53} & \cellbar{0.49}{0.51}{0.26}{0.26}{0.74} & \cellbar{0.07}{0.78}{0.65}{0.28}{0.35} & \cellbar{0.27}{0.60}{0.44}{0.30}{0.56} & \cellbar{0.25}{0.53}{0.51}{0.24}{0.49} & \cellbar{0.06}{0.95}{0.58}{0.36}{0.42} & \cellbar{0.27}{0.83}{0.44}{0.30}{0.56} & 0.77 \\
\textbf{10605} & \cellbar{0.20}{0.88}{0.35}{0.46}{0.65} & \cellbar{0.13}{1.00}{0.35}{0.52}{0.65} & \cellbar{0.47}{0.89}{0.27}{0.27}{0.73} & \cellbar{0.02}{0.83}{0.56}{0.42}{0.44} & \cellbar{0.56}{0.47}{0.30}{0.14}{0.70} & \cellbar{0.07}{0.65}{0.39}{0.54}{0.61} & \cellbar{0.04}{0.85}{0.35}{0.61}{0.65} & \cellbar{0.32}{0.76}{0.66}{0.02}{0.34} & \cellbar{0.20}{0.72}{0.43}{0.38}{0.57} & \cellbar{0.11}{0.97}{0.36}{0.53}{0.64} & \cellbar{0.17}{0.72}{0.40}{0.44}{0.60} & \cellbar{0.42}{0.96}{0.42}{0.17}{0.58} & 0.81 \\
\textbf{14049} & \cellbar{0.22}{0.98}{0.44}{0.35}{0.56} & \cellbar{0.10}{0.59}{0.34}{0.56}{0.66} & \cellbar{0.28}{0.83}{0.41}{0.32}{0.59} & \cellbar{0.02}{0.99}{0.57}{0.41}{0.43} & \cellbar{0.40}{0.51}{0.34}{0.27}{0.66} & \cellbar{0.06}{0.95}{0.18}{0.76}{0.82} & \cellbar{0.47}{0.65}{0.38}{0.16}{0.62} & \cellbar{0.32}{0.75}{0.56}{0.12}{0.44} & \cellbar{0.21}{0.89}{0.50}{0.29}{0.50} & \cellbar{0.12}{0.66}{0.36}{0.52}{0.64} & \cellbar{0.28}{0.67}{0.38}{0.35}{0.62} & \cellbar{0.54}{1.00}{0.38}{0.08}{0.62} & 0.79 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Value steering using SAE features for the {Gemma-2B-IT} model. For each pair of steering feature and value dimension, the cell shows the stimulation ratio in blue, the suppression ratio in yellow, and the maintenance ratio in blank, which are estimated from the training data. The numbers in the cell represent the distance between the actual ratios in the testing data and expected ratios.}

\label{table: sae-steering-gemma}
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} *{12}{>{\centering\arraybackslash}m{1cm}}>{\centering\arraybackslash}m{1cm}}
\toprule
\rotatebox{90}{\textbf{Value}} & \rotatebox{90}{\textbf{Achievement}} & \rotatebox{90}{\textbf{Aesthetic}} & \rotatebox{90}{\textbf{Anxiety Disorder}} & \rotatebox{90}{\textbf{Breadth of Interest}} & \rotatebox{90}{\textbf{Empathy}} & \rotatebox{90}{\textbf{Organization}} & \rotatebox{90}{\textbf{Political}} & \rotatebox{90}{\textbf{Positive coping}} & \rotatebox{90}{\textbf{Religious}} & \rotatebox{90}{\textbf{Resilience}} & \rotatebox{90}{\textbf{Social Complexity}} & \rotatebox{90}{\textbf{Uncertainty Avoidance}} & \textbf{AVG} \\
\midrule
\textbf{428} & \cellbar{0.19}{0.91}{0.58}{0.23}{0.42} & \cellbar{0.15}{0.96}{0.62}{0.23}{0.38} & \cellbar{0.46}{0.89}{0.36}{0.19}{0.64} & \cellbar{0.03}{0.93}{0.65}{0.32}{0.35} & \cellbar{0.23}{0.61}{0.49}{0.29}{0.51} & \cellbar{0.57}{0.57}{0.36}{0.07}{0.64} & \cellbar{0.49}{0.65}{0.40}{0.12}{0.60} & \cellbar{0.30}{0.97}{0.62}{0.08}{0.38} & \cellbar{0.20}{0.92}{0.58}{0.22}{0.42} & \cellbar{0.22}{0.97}{0.59}{0.19}{0.41} & \cellbar{0.17}{0.89}{0.52}{0.31}{0.48} & \cellbar{0.45}{0.89}{0.49}{0.07}{0.51} & 0.85 \\
\textbf{1312} & \cellbar{0.14}{0.96}{0.60}{0.26}{0.40} & \cellbar{0.21}{0.96}{0.65}{0.14}{0.35} & \cellbar{0.77}{0.99}{0.08}{0.15}{0.92} & \cellbar{0.00}{0.41}{0.29}{0.71}{0.71} & \cellbar{0.16}{0.80}{0.38}{0.47}{0.62} & \cellbar{0.09}{0.95}{0.64}{0.27}{0.36} & \cellbar{0.23}{0.91}{0.58}{0.19}{0.42} & \cellbar{0.26}{0.67}{0.68}{0.06}{0.32} & \cellbar{0.55}{0.65}{0.41}{0.04}{0.59} & \cellbar{0.15}{0.90}{0.52}{0.33}{0.48} & \cellbar{0.07}{0.45}{0.18}{0.75}{0.82} & \cellbar{0.71}{0.94}{0.29}{0.00}{0.71} & 0.80 \\
\textbf{1975} & \cellbar{0.11}{0.86}{0.66}{0.23}{0.34} & \cellbar{0.18}{0.81}{0.42}{0.41}{0.58} & \cellbar{0.25}{0.87}{0.41}{0.35}{0.59} & \cellbar{0.05}{0.97}{0.71}{0.24}{0.29} & \cellbar{0.02}{0.69}{0.35}{0.63}{0.65} & \cellbar{0.47}{0.69}{0.39}{0.15}{0.61} & \cellbar{0.12}{0.78}{0.50}{0.39}{0.50} & \cellbar{0.66}{0.91}{0.23}{0.11}{0.77} & \cellbar{0.18}{0.69}{0.48}{0.35}{0.52} & \cellbar{0.12}{0.71}{0.70}{0.18}{0.30} & \cellbar{0.21}{0.72}{0.69}{0.10}{0.31} & \cellbar{0.25}{0.99}{0.64}{0.11}{0.36} & 0.81 \\
\textbf{3183} & \cellbar{0.19}{0.95}{0.22}{0.59}{0.78} & \cellbar{0.58}{0.66}{0.16}{0.26}{0.84} & \cellbar{0.68}{0.97}{0.18}{0.14}{0.82} & \cellbar{0.16}{0.82}{0.35}{0.50}{0.65} & \cellbar{0.20}{0.97}{0.20}{0.60}{0.80} & \cellbar{0.22}{0.78}{0.36}{0.43}{0.64} & \cellbar{0.40}{0.73}{0.24}{0.37}{0.76} & \cellbar{0.33}{0.87}{0.35}{0.33}{0.65} & \cellbar{0.76}{0.16}{0.16}{0.08}{0.84} & \cellbar{0.46}{0.55}{0.48}{0.07}{0.52} & \cellbar{0.13}{0.57}{0.36}{0.51}{0.64} & \cellbar{0.67}{0.94}{0.21}{0.12}{0.79} & 0.75 \\
\textbf{4752} & \cellbar{0.16}{0.97}{0.35}{0.50}{0.65} & \cellbar{0.08}{0.64}{0.41}{0.51}{0.59} & \cellbar{0.64}{0.38}{0.28}{0.08}{0.72} & \cellbar{0.20}{1.00}{0.53}{0.27}{0.47} & \cellbar{0.43}{0.69}{0.27}{0.31}{0.73} & \cellbar{0.29}{0.73}{0.42}{0.30}{0.58} & \cellbar{0.21}{0.76}{0.43}{0.37}{0.57} & \cellbar{0.44}{0.87}{0.45}{0.12}{0.55} & \cellbar{0.07}{0.86}{0.58}{0.35}{0.42} & \cellbar{0.08}{1.00}{0.25}{0.67}{0.75} & \cellbar{0.09}{0.99}{0.14}{0.77}{0.86} & \cellbar{0.25}{0.91}{0.47}{0.29}{0.53} & 0.81 \\
\textbf{6216} & \cellbar{0.22}{0.98}{0.61}{0.17}{0.39} & \cellbar{0.06}{0.80}{0.50}{0.45}{0.50} & \cellbar{0.64}{0.84}{0.15}{0.21}{0.85} & \cellbar{0.00}{0.49}{0.32}{0.68}{0.68} & \cellbar{0.16}{0.97}{0.50}{0.35}{0.50} & \cellbar{0.29}{0.92}{0.62}{0.09}{0.38} & \cellbar{0.14}{0.94}{0.65}{0.21}{0.35} & \cellbar{0.27}{0.80}{0.65}{0.08}{0.35} & \cellbar{0.06}{0.99}{0.79}{0.15}{0.21} & \cellbar{0.18}{0.83}{0.50}{0.32}{0.50} & \cellbar{0.20}{0.91}{0.51}{0.29}{0.49} & \cellbar{0.29}{0.90}{0.60}{0.11}{0.40} & 0.87 \\
\textbf{6619} & \cellbar{0.25}{0.89}{0.52}{0.23}{0.48} & \cellbar{0.18}{0.82}{0.58}{0.24}{0.42} & \cellbar{0.21}{0.56}{0.27}{0.52}{0.73} & \cellbar{0.02}{0.92}{0.68}{0.30}{0.32} & \cellbar{0.10}{0.76}{0.33}{0.57}{0.67} & \cellbar{0.39}{0.81}{0.46}{0.16}{0.54} & \cellbar{0.10}{0.58}{0.38}{0.52}{0.62} & \cellbar{0.62}{0.99}{0.32}{0.06}{0.68} & \cellbar{0.22}{0.89}{0.40}{0.39}{0.60} & \cellbar{0.26}{0.60}{0.63}{0.11}{0.37} & \cellbar{0.46}{0.80}{0.41}{0.14}{0.59} & \cellbar{0.57}{0.76}{0.40}{0.03}{0.60} & 0.78 \\
\textbf{8387} & \cellbar{0.25}{0.83}{0.49}{0.27}{0.51} & \cellbar{0.30}{1.00}{0.49}{0.22}{0.51} & \cellbar{0.15}{0.66}{0.50}{0.35}{0.50} & \cellbar{0.11}{0.98}{0.62}{0.27}{0.38} & \cellbar{0.60}{0.91}{0.33}{0.07}{0.67} & \cellbar{0.37}{0.76}{0.45}{0.19}{0.55} & \cellbar{0.40}{0.72}{0.35}{0.26}{0.65} & \cellbar{0.38}{0.99}{0.43}{0.20}{0.57} & \cellbar{0.14}{0.90}{0.34}{0.52}{0.66} & \cellbar{0.27}{0.89}{0.51}{0.22}{0.49} & \cellbar{0.13}{0.63}{0.50}{0.37}{0.50} & \cellbar{0.34}{1.00}{0.63}{0.03}{0.37} & 0.86 \\
\textbf{10096} & \cellbar{0.30}{0.64}{0.44}{0.27}{0.56} & \cellbar{0.27}{0.73}{0.36}{0.38}{0.64} & \cellbar{0.34}{0.92}{0.30}{0.37}{0.70} & \cellbar{0.41}{0.97}{0.45}{0.15}{0.55} & \cellbar{0.60}{1.00}{0.26}{0.14}{0.74} & \cellbar{0.34}{0.86}{0.47}{0.20}{0.53} & \cellbar{0.49}{0.53}{0.26}{0.26}{0.74} & \cellbar{0.07}{0.81}{0.65}{0.28}{0.35} & \cellbar{0.27}{0.63}{0.44}{0.30}{0.56} & \cellbar{0.25}{0.53}{0.51}{0.24}{0.49} & \cellbar{0.06}{0.93}{0.58}{0.36}{0.42} & \cellbar{0.27}{0.81}{0.44}{0.30}{0.56} & 0.78 \\
\textbf{10605} & \cellbar{0.20}{0.87}{0.35}{0.46}{0.65} & \cellbar{0.13}{0.99}{0.35}{0.52}{0.65} & \cellbar{0.47}{0.91}{0.27}{0.27}{0.73} & \cellbar{0.02}{0.83}{0.56}{0.42}{0.44} & \cellbar{0.56}{0.52}{0.30}{0.14}{0.70} & \cellbar{0.07}{0.68}{0.39}{0.54}{0.61} & \cellbar{0.04}{0.84}{0.35}{0.61}{0.65} & \cellbar{0.32}{0.79}{0.66}{0.02}{0.34} & \cellbar{0.20}{0.72}{0.43}{0.38}{0.57} & \cellbar{0.11}{0.96}{0.36}{0.53}{0.64} & \cellbar{0.17}{0.73}{0.40}{0.44}{0.60} & \cellbar{0.42}{0.96}{0.42}{0.17}{0.58} & 0.82 \\
\textbf{14049} & \cellbar{0.22}{0.98}{0.44}{0.35}{0.56} & \cellbar{0.10}{0.60}{0.34}{0.56}{0.66} & \cellbar{0.28}{0.85}{0.41}{0.32}{0.59} & \cellbar{0.02}{0.99}{0.57}{0.41}{0.43} & \cellbar{0.40}{0.53}{0.34}{0.27}{0.66} & \cellbar{0.06}{0.96}{0.18}{0.76}{0.82} & \cellbar{0.47}{0.65}{0.38}{0.16}{0.62} & \cellbar{0.32}{0.74}{0.56}{0.12}{0.44} & \cellbar{0.21}{0.89}{0.50}{0.29}{0.50} & \cellbar{0.12}{0.65}{0.36}{0.52}{0.64} & \cellbar{0.28}{0.69}{0.38}{0.35}{0.62} & \cellbar{0.54}{1.00}{0.38}{0.08}{0.62} & 0.79 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Value steering using SAE features for the {Llama3-8B-IT} model. For each pair of steering feature and value dimension, the cell shows the stimulation ratio in blue, the suppression ratio in yellow, and the maintenance ratio in blank, which are estimated from the training data. The numbers in the cell represent the distance between the actual ratios in the testing data and expected ratios.}

\label{table: sae-steering-gemma}
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} *{21}{>{\centering\arraybackslash}m{1cm}}>{\centering\arraybackslash}m{1cm}}
\toprule
\rotatebox{90}{\textbf{Value}} & \rotatebox{90}{\textbf{Affiliation}} & \rotatebox{90}{\textbf{Assertiveness}} & \rotatebox{90}{\textbf{Behavioral Inhibition System}} & \rotatebox{90}{\textbf{Breadth of Interest}} & \rotatebox{90}{\textbf{Emotional Expression}} & \rotatebox{90}{\textbf{Empathy}} & \rotatebox{90}{\textbf{Extraversion}} & \rotatebox{90}{\textbf{Nurturance}} & \rotatebox{90}{\textbf{Poise}} & \rotatebox{90}{\textbf{Positive Expressivity}} & \rotatebox{90}{\textbf{Preference for Order and Structure}} & \rotatebox{90}{\textbf{Psychosocial flourishing}} & \rotatebox{90}{\textbf{Satisfaction with life}} & \rotatebox{90}{\textbf{Sociability}} & \rotatebox{90}{\textbf{Social}} & \rotatebox{90}{\textbf{Social Confidence}} & \rotatebox{90}{\textbf{Social Withdrawal}} & \rotatebox{90}{\textbf{Sympathy}} & \rotatebox{90}{\textbf{Tenderness}} & \rotatebox{90}{\textbf{Theoretical}} & \rotatebox{90}{\textbf{Understanding}} & \textbf{AVG} \\
\midrule
\textbf{1897} & \cellbar{0.06}{1.00}{0.84}{0.10}{0.16} & \cellbar{0.22}{0.99}{0.50}{0.28}{0.50} & \cellbar{0.11}{0.97}{0.76}{0.13}{0.24} & \cellbar{0.16}{1.00}{0.76}{0.08}{0.24} & \cellbar{0.09}{0.96}{0.75}{0.16}{0.25} & \cellbar{0.22}{0.99}{0.65}{0.13}{0.35} & \cellbar{0.23}{0.98}{0.62}{0.15}{0.38} & \cellbar{0.09}{0.99}{0.81}{0.10}{0.19} & \cellbar{0.07}{1.00}{0.87}{0.06}{0.13} & \cellbar{0.12}{1.00}{0.72}{0.16}{0.28} & \cellbar{0.24}{0.99}{0.50}{0.26}{0.50} & \cellbar{0.35}{1.00}{0.58}{0.07}{0.42} & \cellbar{0.16}{0.97}{0.64}{0.20}{0.36} & \cellbar{0.27}{1.00}{0.40}{0.34}{0.60} & \cellbar{0.51}{1.00}{0.25}{0.24}{0.75} & \cellbar{0.17}{0.99}{0.69}{0.14}{0.31} & \cellbar{0.18}{0.94}{0.75}{0.07}{0.25} & \cellbar{0.11}{1.00}{0.83}{0.06}{0.17} & \cellbar{0.06}{1.00}{0.83}{0.11}{0.17} & \cellbar{0.41}{0.99}{0.28}{0.32}{0.72} & \cellbar{0.11}{1.00}{0.85}{0.04}{0.15} & 0.99 \\
\textbf{2246} & \cellbar{0.13}{0.96}{0.55}{0.32}{0.45} & \cellbar{0.13}{0.99}{0.22}{0.65}{0.78} & \cellbar{0.27}{0.99}{0.38}{0.36}{0.62} & \cellbar{0.24}{1.00}{0.59}{0.17}{0.41} & \cellbar{0.17}{0.92}{0.29}{0.54}{0.71} & \cellbar{0.21}{0.98}{0.39}{0.41}{0.61} & \cellbar{0.25}{0.99}{0.16}{0.59}{0.84} & \cellbar{0.26}{0.98}{0.48}{0.27}{0.52} & \cellbar{0.27}{0.94}{0.63}{0.10}{0.37} & \cellbar{0.40}{0.97}{0.42}{0.19}{0.58} & \cellbar{0.39}{0.99}{0.22}{0.40}{0.78} & \cellbar{0.32}{0.95}{0.38}{0.31}{0.62} & \cellbar{0.33}{1.00}{0.44}{0.24}{0.56} & \cellbar{0.28}{0.97}{0.27}{0.46}{0.73} & \cellbar{0.24}{0.99}{0.12}{0.64}{0.88} & \cellbar{0.23}{0.96}{0.27}{0.50}{0.73} & \cellbar{0.25}{0.97}{0.54}{0.21}{0.46} & \cellbar{0.12}{1.00}{0.71}{0.17}{0.29} & \cellbar{0.26}{0.99}{0.47}{0.28}{0.53} & \cellbar{0.15}{0.97}{0.20}{0.65}{0.80} & \cellbar{0.19}{0.99}{0.67}{0.14}{0.33} & 0.98 \\
\textbf{2509} & \cellbar{0.21}{0.98}{0.47}{0.33}{0.53} & \cellbar{0.29}{0.95}{0.23}{0.49}{0.77} & \cellbar{0.45}{0.99}{0.32}{0.24}{0.68} & \cellbar{0.36}{0.96}{0.46}{0.19}{0.54} & \cellbar{0.19}{0.98}{0.62}{0.19}{0.38} & \cellbar{0.80}{0.99}{0.11}{0.09}{0.89} & \cellbar{0.43}{0.96}{0.25}{0.33}{0.75} & \cellbar{0.33}{0.98}{0.45}{0.23}{0.55} & \cellbar{0.23}{1.00}{0.65}{0.12}{0.35} & \cellbar{0.37}{0.98}{0.37}{0.27}{0.63} & \cellbar{0.17}{0.98}{0.11}{0.72}{0.89} & \cellbar{0.58}{0.99}{0.31}{0.11}{0.69} & \cellbar{0.15}{0.97}{0.36}{0.50}{0.64} & \cellbar{0.39}{0.99}{0.19}{0.43}{0.81} & \cellbar{0.70}{1.00}{0.12}{0.18}{0.88} & \cellbar{0.30}{0.97}{0.36}{0.35}{0.64} & \cellbar{0.29}{0.96}{0.52}{0.19}{0.48} & \cellbar{0.25}{1.00}{0.61}{0.14}{0.39} & \cellbar{0.26}{0.99}{0.35}{0.40}{0.65} & \cellbar{0.12}{1.00}{0.11}{0.77}{0.89} & \cellbar{0.34}{0.94}{0.39}{0.28}{0.61} & 0.98 \\
\textbf{20141} & \cellbar{0.19}{0.97}{0.19}{0.62}{0.81} & \cellbar{0.59}{0.98}{0.13}{0.28}{0.87} & \cellbar{0.54}{0.99}{0.18}{0.28}{0.82} & \cellbar{0.20}{1.00}{0.31}{0.49}{0.69} & \cellbar{0.25}{0.99}{0.30}{0.45}{0.70} & \cellbar{0.05}{1.00}{0.10}{0.85}{0.90} & \cellbar{0.61}{0.99}{0.15}{0.24}{0.85} & \cellbar{0.44}{0.98}{0.19}{0.37}{0.81} & \cellbar{0.18}{0.98}{0.23}{0.59}{0.77} & \cellbar{0.20}{0.98}{0.06}{0.74}{0.94} & \cellbar{0.36}{0.98}{0.15}{0.49}{0.85} & \cellbar{0.42}{1.00}{0.24}{0.34}{0.76} & \cellbar{0.26}{1.00}{0.33}{0.41}{0.67} & \cellbar{0.34}{0.97}{0.14}{0.52}{0.86} & \cellbar{0.05}{0.99}{0.08}{0.87}{0.92} & \cellbar{0.37}{0.96}{0.16}{0.47}{0.84} & \cellbar{0.45}{0.93}{0.28}{0.27}{0.72} & \cellbar{0.06}{0.99}{0.11}{0.83}{0.89} & \cellbar{0.60}{0.98}{0.19}{0.21}{0.81} & \cellbar{0.11}{1.00}{0.08}{0.81}{0.92} & \cellbar{0.04}{1.00}{0.21}{0.75}{0.79} & 0.98 \\
\textbf{41929} & \cellbar{0.19}{0.97}{0.36}{0.46}{0.64} & \cellbar{0.35}{0.99}{0.24}{0.42}{0.76} & \cellbar{0.37}{0.91}{0.32}{0.32}{0.68} & \cellbar{0.18}{0.99}{0.56}{0.26}{0.44} & \cellbar{0.30}{0.99}{0.53}{0.17}{0.47} & \cellbar{0.36}{0.99}{0.46}{0.19}{0.54} & \cellbar{0.47}{0.97}{0.22}{0.32}{0.78} & \cellbar{0.51}{0.98}{0.43}{0.06}{0.57} & \cellbar{0.23}{0.98}{0.58}{0.19}{0.42} & \cellbar{0.28}{0.93}{0.53}{0.19}{0.47} & \cellbar{0.31}{0.97}{0.42}{0.28}{0.58} & \cellbar{0.49}{0.96}{0.23}{0.29}{0.77} & \cellbar{0.20}{1.00}{0.43}{0.38}{0.57} & \cellbar{0.32}{0.99}{0.28}{0.41}{0.72} & \cellbar{0.60}{1.00}{0.18}{0.22}{0.82} & \cellbar{0.41}{0.97}{0.27}{0.33}{0.73} & \cellbar{0.27}{0.98}{0.57}{0.16}{0.43} & \cellbar{0.07}{0.99}{0.70}{0.23}{0.30} & \cellbar{0.59}{1.00}{0.26}{0.15}{0.74} & \cellbar{0.51}{0.99}{0.18}{0.31}{0.82} & \cellbar{0.27}{0.98}{0.65}{0.08}{0.35} & 0.98 \\
\textbf{48321} & \cellbar{0.12}{0.99}{0.34}{0.54}{0.66} & \cellbar{0.40}{0.99}{0.21}{0.40}{0.79} & \cellbar{0.51}{0.92}{0.25}{0.24}{0.75} & \cellbar{0.13}{1.00}{0.39}{0.49}{0.61} & \cellbar{0.31}{1.00}{0.44}{0.26}{0.56} & \cellbar{0.16}{0.98}{0.18}{0.66}{0.82} & \cellbar{0.38}{0.96}{0.26}{0.37}{0.74} & \cellbar{0.30}{0.99}{0.38}{0.33}{0.62} & \cellbar{0.23}{1.00}{0.46}{0.32}{0.54} & \cellbar{0.32}{1.00}{0.24}{0.45}{0.76} & \cellbar{0.28}{0.97}{0.23}{0.50}{0.77} & \cellbar{0.28}{0.97}{0.27}{0.46}{0.73} & \cellbar{0.32}{0.91}{0.35}{0.34}{0.65} & \cellbar{0.31}{1.00}{0.16}{0.53}{0.84} & \cellbar{0.14}{1.00}{0.11}{0.75}{0.89} & \cellbar{0.31}{0.94}{0.21}{0.49}{0.79} & \cellbar{0.29}{0.99}{0.53}{0.18}{0.47} & \cellbar{0.16}{0.89}{0.56}{0.28}{0.44} & \cellbar{0.39}{0.99}{0.27}{0.35}{0.73} & \cellbar{0.05}{1.00}{0.04}{0.91}{0.96} & \cellbar{0.17}{0.98}{0.40}{0.44}{0.60} & 0.97 \\
\textbf{49202} & \cellbar{0.21}{0.97}{0.57}{0.22}{0.43} & \cellbar{0.36}{0.95}{0.26}{0.39}{0.74} & \cellbar{0.53}{0.99}{0.30}{0.17}{0.70} & \cellbar{0.21}{0.99}{0.61}{0.18}{0.39} & \cellbar{0.26}{0.98}{0.63}{0.11}{0.37} & \cellbar{0.52}{0.97}{0.23}{0.25}{0.77} & \cellbar{0.33}{0.94}{0.22}{0.46}{0.78} & \cellbar{0.25}{1.00}{0.53}{0.22}{0.47} & \cellbar{0.18}{1.00}{0.52}{0.30}{0.48} & \cellbar{0.33}{0.98}{0.42}{0.26}{0.58} & \cellbar{0.30}{0.95}{0.27}{0.44}{0.73} & \cellbar{0.59}{0.99}{0.32}{0.09}{0.68} & \cellbar{0.39}{0.95}{0.36}{0.26}{0.64} & \cellbar{0.66}{1.00}{0.18}{0.16}{0.82} & \cellbar{0.50}{0.93}{0.19}{0.32}{0.81} & \cellbar{0.33}{0.99}{0.33}{0.35}{0.67} & \cellbar{0.19}{0.98}{0.64}{0.17}{0.36} & \cellbar{0.06}{0.94}{0.38}{0.56}{0.62} & \cellbar{0.23}{1.00}{0.41}{0.37}{0.59} & \cellbar{0.35}{0.97}{0.24}{0.42}{0.76} & \cellbar{0.27}{1.00}{0.60}{0.13}{0.40} & 0.97 \\
\textbf{58305} & \cellbar{0.08}{0.98}{0.66}{0.26}{0.34} & \cellbar{0.33}{0.99}{0.36}{0.32}{0.64} & \cellbar{0.25}{0.99}{0.51}{0.24}{0.49} & \cellbar{0.23}{0.99}{0.70}{0.07}{0.30} & \cellbar{0.24}{0.98}{0.57}{0.19}{0.43} & \cellbar{0.24}{0.98}{0.51}{0.25}{0.49} & \cellbar{0.41}{0.97}{0.30}{0.30}{0.70} & \cellbar{0.22}{1.00}{0.71}{0.07}{0.29} & \cellbar{0.13}{1.00}{0.78}{0.09}{0.22} & \cellbar{0.23}{0.97}{0.59}{0.18}{0.41} & \cellbar{0.28}{0.86}{0.43}{0.30}{0.57} & \cellbar{0.36}{0.99}{0.37}{0.28}{0.63} & \cellbar{0.33}{0.99}{0.49}{0.19}{0.51} & \cellbar{0.20}{0.99}{0.38}{0.43}{0.62} & \cellbar{0.45}{0.99}{0.16}{0.40}{0.84} & \cellbar{0.33}{0.90}{0.43}{0.25}{0.57} & \cellbar{0.18}{1.00}{0.70}{0.12}{0.30} & \cellbar{0.13}{0.99}{0.72}{0.15}{0.28} & \cellbar{0.26}{0.99}{0.67}{0.07}{0.33} & \cellbar{0.51}{0.94}{0.22}{0.27}{0.78} & \cellbar{0.20}{0.99}{0.72}{0.08}{0.28} & 0.97 \\
\textbf{63905} & \cellbar{0.12}{0.97}{0.30}{0.58}{0.70} & \cellbar{0.67}{0.99}{0.10}{0.23}{0.90} & \cellbar{0.38}{0.96}{0.32}{0.31}{0.68} & \cellbar{0.28}{0.98}{0.34}{0.39}{0.66} & \cellbar{0.11}{1.00}{0.46}{0.44}{0.54} & \cellbar{0.39}{0.89}{0.22}{0.40}{0.78} & \cellbar{0.82}{0.99}{0.05}{0.13}{0.95} & \cellbar{0.56}{0.93}{0.36}{0.08}{0.64} & \cellbar{0.19}{0.97}{0.40}{0.42}{0.60} & \cellbar{0.31}{0.98}{0.41}{0.29}{0.59} & \cellbar{0.38}{0.98}{0.23}{0.40}{0.77} & \cellbar{0.50}{0.89}{0.24}{0.27}{0.76} & \cellbar{0.77}{0.99}{0.11}{0.12}{0.89} & \cellbar{0.33}{0.98}{0.27}{0.41}{0.73} & \cellbar{0.84}{1.00}{0.07}{0.09}{0.93} & \cellbar{0.42}{0.97}{0.31}{0.28}{0.69} & \cellbar{0.43}{0.97}{0.37}{0.21}{0.63} & \cellbar{0.34}{0.97}{0.44}{0.23}{0.56} & \cellbar{0.85}{1.00}{0.12}{0.03}{0.88} & \cellbar{0.43}{0.93}{0.13}{0.45}{0.87} & \cellbar{0.23}{0.94}{0.36}{0.42}{0.64} & 0.97 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Value steering using SAE features for the {Llama3-8B-IT} model. For each pair of steering feature and value dimension, the cell shows the stimulation ratio in blue, the suppression ratio in yellow, and the maintenance ratio in blank, which are estimated from the training data. The numbers in the cell represent the distance between the actual ratios in the testing data and expected ratios.}

\label{table: sae-steering-Llama3-8B-IT}
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} *{17}{>{\centering\arraybackslash}m{1cm}}>{\centering\arraybackslash}m{1cm}}
\toprule
\rotatebox{90}{\textbf{Value}} & \rotatebox{90}{\textbf{Achievement}} & \rotatebox{90}{\textbf{Aesthetic}} & \rotatebox{90}{\textbf{Anxiety Disorder}} & \rotatebox{90}{\textbf{Breadth of Interest}} & \rotatebox{90}{\textbf{Economic}} & \rotatebox{90}{\textbf{Empathy}} & \rotatebox{90}{\textbf{Organization}} & \rotatebox{90}{\textbf{Political}} & \rotatebox{90}{\textbf{Positive coping}} & \rotatebox{90}{\textbf{Religious}} & \rotatebox{90}{\textbf{Resilience}} & \rotatebox{90}{\textbf{Social}} & \rotatebox{90}{\textbf{Social Complexity}} & \rotatebox{90}{\textbf{Social Cynicism}} & \rotatebox{90}{\textbf{Theoretical}} & \rotatebox{90}{\textbf{Uncertainty Avoidance}} & \rotatebox{90}{\textbf{Understanding}} & \textbf{AVG} \\
\midrule
\textbf{1897} & \cellbar{0.05}{0.99}{0.78}{0.16}{0.22} & \cellbar{0.01}{0.72}{0.91}{0.08}{0.09} & \cellbar{0.15}{0.80}{0.80}{0.05}{0.20} & \cellbar{0.05}{0.92}{0.88}{0.07}{0.12} & \cellbar{0.19}{0.99}{0.74}{0.07}{0.26} & \cellbar{0.03}{0.99}{0.97}{0.00}{0.03} & \cellbar{0.12}{0.99}{0.85}{0.03}{0.15} & \cellbar{0.11}{0.98}{0.80}{0.09}{0.20} & \cellbar{0.09}{0.99}{0.78}{0.12}{0.22} & \cellbar{0.07}{0.95}{0.85}{0.08}{0.15} & \cellbar{0.00}{0.98}{1.00}{0.00}{0.00} & \cellbar{0.11}{0.47}{0.81}{0.08}{0.19} & \cellbar{0.00}{0.95}{0.96}{0.04}{0.04} & \cellbar{0.01}{1.00}{0.95}{0.04}{0.05} & \cellbar{0.01}{0.91}{0.96}{0.03}{0.04} & \cellbar{0.15}{0.98}{0.73}{0.12}{0.27} & \cellbar{0.05}{0.99}{0.92}{0.03}{0.08} & 0.92 \\
\textbf{2246} & \cellbar{0.09}{0.93}{0.62}{0.28}{0.38} & \cellbar{0.12}{0.70}{0.46}{0.42}{0.54} & \cellbar{0.22}{0.97}{0.61}{0.18}{0.39} & \cellbar{0.16}{0.96}{0.78}{0.05}{0.22} & \cellbar{0.19}{0.95}{0.59}{0.22}{0.41} & \cellbar{0.05}{0.44}{0.84}{0.11}{0.16} & \cellbar{0.12}{0.98}{0.76}{0.12}{0.24} & \cellbar{0.11}{0.93}{0.50}{0.39}{0.50} & \cellbar{0.15}{0.92}{0.55}{0.30}{0.45} & \cellbar{0.16}{0.82}{0.61}{0.23}{0.39} & \cellbar{0.05}{0.84}{0.82}{0.12}{0.18} & \cellbar{0.05}{0.68}{0.41}{0.54}{0.59} & \cellbar{0.16}{0.94}{0.64}{0.20}{0.36} & \cellbar{0.11}{0.97}{0.68}{0.22}{0.32} & \cellbar{0.08}{0.95}{0.34}{0.58}{0.66} & \cellbar{0.35}{0.72}{0.35}{0.30}{0.65} & \cellbar{0.04}{1.00}{0.92}{0.04}{0.08} & 0.86 \\
\textbf{2509} & \cellbar{0.15}{0.98}{0.70}{0.15}{0.30} & \cellbar{0.09}{0.71}{0.45}{0.46}{0.55} & \cellbar{0.19}{0.99}{0.58}{0.23}{0.42} & \cellbar{0.20}{0.95}{0.62}{0.18}{0.38} & \cellbar{0.34}{1.00}{0.55}{0.11}{0.45} & \cellbar{0.12}{0.74}{0.69}{0.19}{0.31} & \cellbar{0.26}{0.92}{0.64}{0.11}{0.36} & \cellbar{0.32}{0.64}{0.38}{0.30}{0.62} & \cellbar{0.12}{0.98}{0.57}{0.31}{0.43} & \cellbar{0.19}{0.95}{0.36}{0.45}{0.64} & \cellbar{0.00}{0.79}{0.93}{0.07}{0.07} & \cellbar{0.26}{0.99}{0.36}{0.38}{0.64} & \cellbar{0.39}{0.84}{0.59}{0.01}{0.41} & \cellbar{0.07}{0.97}{0.45}{0.49}{0.55} & \cellbar{0.14}{0.99}{0.27}{0.59}{0.73} & \cellbar{0.28}{0.77}{0.31}{0.41}{0.69} & \cellbar{0.19}{0.86}{0.80}{0.01}{0.20} & 0.89 \\
\textbf{4305} & \cellbar{0.16}{0.90}{0.55}{0.28}{0.45} & \cellbar{0.45}{0.66}{0.20}{0.35}{0.80} & \cellbar{0.30}{0.96}{0.49}{0.22}{0.51} & \cellbar{0.16}{0.93}{0.54}{0.30}{0.46} & \cellbar{0.39}{0.96}{0.28}{0.32}{0.72} & \cellbar{0.01}{0.79}{0.66}{0.32}{0.34} & \cellbar{0.20}{0.93}{0.55}{0.24}{0.45} & \cellbar{0.19}{0.98}{0.28}{0.53}{0.72} & \cellbar{0.34}{0.88}{0.31}{0.35}{0.69} & \cellbar{0.16}{0.77}{0.19}{0.65}{0.81} & \cellbar{0.03}{0.64}{0.49}{0.49}{0.51} & \cellbar{0.16}{1.00}{0.24}{0.59}{0.76} & \cellbar{0.23}{0.80}{0.43}{0.34}{0.57} & \cellbar{0.08}{0.98}{0.34}{0.58}{0.66} & \cellbar{0.15}{0.52}{0.22}{0.64}{0.78} & \cellbar{0.39}{0.52}{0.32}{0.28}{0.68} & \cellbar{0.11}{0.21}{0.89}{0.00}{0.11} & 0.79 \\
\textbf{7754} & \cellbar{0.03}{0.99}{0.11}{0.86}{0.89} & \cellbar{0.35}{0.86}{0.19}{0.46}{0.81} & \cellbar{0.86}{1.00}{0.08}{0.05}{0.92} & \cellbar{0.00}{0.98}{0.03}{0.97}{0.97} & \cellbar{0.38}{0.73}{0.27}{0.35}{0.73} & \cellbar{0.00}{1.00}{0.00}{1.00}{1.00} & \cellbar{0.00}{1.00}{0.00}{1.00}{1.00} & \cellbar{0.65}{0.51}{0.18}{0.18}{0.82} & \cellbar{0.03}{1.00}{0.07}{0.91}{0.93} & \cellbar{0.22}{0.93}{0.23}{0.55}{0.77} & \cellbar{0.00}{0.97}{0.00}{1.00}{1.00} & \cellbar{0.09}{0.94}{0.05}{0.85}{0.95} & \cellbar{0.00}{1.00}{0.00}{1.00}{1.00} & \cellbar{0.99}{0.90}{0.01}{0.00}{0.99} & \cellbar{0.01}{0.79}{0.01}{0.97}{0.99} & \cellbar{0.59}{0.90}{0.12}{0.28}{0.88} & \cellbar{0.00}{1.00}{0.00}{1.00}{1.00} & 0.91 \\
\textbf{8035} & \cellbar{0.01}{0.99}{0.95}{0.04}{0.05} & \cellbar{0.03}{0.97}{0.81}{0.16}{0.19} & \cellbar{0.05}{1.00}{0.91}{0.04}{0.09} & \cellbar{0.03}{0.98}{0.93}{0.04}{0.07} & \cellbar{0.08}{1.00}{0.91}{0.01}{0.09} & \cellbar{0.01}{0.98}{0.95}{0.04}{0.05} & \cellbar{0.04}{1.00}{0.96}{0.00}{0.04} & \cellbar{0.01}{1.00}{0.89}{0.09}{0.11} & \cellbar{0.05}{1.00}{0.91}{0.04}{0.09} & \cellbar{0.08}{1.00}{0.89}{0.03}{0.11} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.01}{0.98}{0.89}{0.09}{0.11} & \cellbar{0.01}{0.98}{0.97}{0.01}{0.03} & \cellbar{0.08}{1.00}{0.88}{0.04}{0.12} & \cellbar{0.03}{0.92}{0.86}{0.11}{0.14} & \cellbar{0.05}{0.96}{0.73}{0.22}{0.27} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & 0.98 \\
\textbf{8546} & \cellbar{0.12}{0.96}{0.70}{0.18}{0.30} & \cellbar{0.20}{0.88}{0.47}{0.32}{0.53} & \cellbar{0.09}{0.94}{0.66}{0.24}{0.34} & \cellbar{0.14}{0.99}{0.66}{0.20}{0.34} & \cellbar{0.26}{0.94}{0.65}{0.09}{0.35} & \cellbar{0.05}{0.93}{0.86}{0.08}{0.14} & \cellbar{0.22}{0.96}{0.76}{0.03}{0.24} & \cellbar{0.19}{0.94}{0.53}{0.28}{0.47} & \cellbar{0.27}{0.98}{0.57}{0.16}{0.43} & \cellbar{0.16}{1.00}{0.50}{0.34}{0.50} & \cellbar{0.03}{0.96}{0.92}{0.05}{0.08} & \cellbar{0.12}{0.88}{0.50}{0.38}{0.50} & \cellbar{0.07}{0.89}{0.64}{0.30}{0.36} & \cellbar{0.27}{0.96}{0.58}{0.15}{0.42} & \cellbar{0.05}{0.84}{0.59}{0.35}{0.41} & \cellbar{0.53}{0.57}{0.27}{0.20}{0.73} & \cellbar{0.07}{1.00}{0.89}{0.04}{0.11} & 0.92 \\
\textbf{9332} & \cellbar{0.41}{0.89}{0.32}{0.27}{0.68} & \cellbar{0.43}{0.97}{0.15}{0.42}{0.85} & \cellbar{0.39}{0.83}{0.20}{0.41}{0.80} & \cellbar{0.09}{0.49}{0.27}{0.64}{0.73} & \cellbar{0.47}{0.96}{0.35}{0.18}{0.65} & \cellbar{0.09}{0.97}{0.23}{0.68}{0.77} & \cellbar{0.28}{0.88}{0.42}{0.30}{0.58} & \cellbar{0.54}{0.93}{0.27}{0.19}{0.73} & \cellbar{0.45}{0.77}{0.34}{0.22}{0.66} & \cellbar{0.51}{0.98}{0.28}{0.20}{0.72} & \cellbar{0.30}{0.80}{0.49}{0.22}{0.51} & \cellbar{0.28}{0.79}{0.22}{0.50}{0.78} & \cellbar{0.31}{0.75}{0.30}{0.39}{0.70} & \cellbar{0.78}{0.89}{0.12}{0.09}{0.88} & \cellbar{0.41}{0.84}{0.19}{0.41}{0.81} & \cellbar{0.61}{0.70}{0.16}{0.23}{0.84} & \cellbar{0.12}{0.99}{0.46}{0.42}{0.54} & 0.85 \\
\textbf{12477} & \cellbar{0.04}{1.00}{0.92}{0.04}{0.08} & \cellbar{0.07}{1.00}{0.81}{0.12}{0.19} & \cellbar{0.04}{1.00}{0.91}{0.05}{0.09} & \cellbar{0.05}{1.00}{0.91}{0.04}{0.09} & \cellbar{0.23}{0.95}{0.74}{0.03}{0.26} & \cellbar{0.03}{0.99}{0.95}{0.03}{0.05} & \cellbar{0.07}{1.00}{0.93}{0.00}{0.07} & \cellbar{0.08}{0.99}{0.82}{0.09}{0.18} & \cellbar{0.07}{0.99}{0.89}{0.04}{0.11} & \cellbar{0.07}{1.00}{0.81}{0.12}{0.19} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.07}{0.96}{0.89}{0.04}{0.11} & \cellbar{0.03}{1.00}{0.93}{0.04}{0.07} & \cellbar{0.07}{1.00}{0.89}{0.04}{0.11} & \cellbar{0.04}{1.00}{0.86}{0.09}{0.14} & \cellbar{0.04}{0.96}{0.78}{0.18}{0.22} & \cellbar{0.01}{1.00}{0.99}{0.00}{0.01} & 0.99 \\
\textbf{13033} & \cellbar{0.11}{0.48}{0.15}{0.74}{0.85} & \cellbar{0.42}{0.90}{0.22}{0.36}{0.78} & \cellbar{0.51}{1.00}{0.20}{0.28}{0.80} & \cellbar{0.09}{0.50}{0.14}{0.77}{0.86} & \cellbar{0.34}{0.97}{0.16}{0.50}{0.84} & \cellbar{0.05}{0.92}{0.14}{0.81}{0.86} & \cellbar{0.09}{0.99}{0.09}{0.81}{0.91} & \cellbar{0.61}{0.82}{0.15}{0.24}{0.85} & \cellbar{0.23}{0.99}{0.16}{0.61}{0.84} & \cellbar{0.35}{1.00}{0.11}{0.54}{0.89} & \cellbar{0.04}{1.00}{0.12}{0.84}{0.88} & \cellbar{0.31}{0.97}{0.19}{0.50}{0.81} & \cellbar{0.11}{0.99}{0.11}{0.78}{0.89} & \cellbar{0.54}{0.69}{0.19}{0.27}{0.81} & \cellbar{0.31}{0.91}{0.14}{0.55}{0.86} & \cellbar{0.46}{0.98}{0.16}{0.38}{0.84} & \cellbar{0.12}{0.98}{0.18}{0.70}{0.82} & 0.89 \\
\textbf{20141} & \cellbar{0.36}{0.92}{0.45}{0.19}{0.55} & \cellbar{0.39}{0.68}{0.22}{0.39}{0.78} & \cellbar{0.39}{0.99}{0.32}{0.28}{0.68} & \cellbar{0.15}{0.89}{0.50}{0.35}{0.50} & \cellbar{0.28}{0.94}{0.47}{0.24}{0.53} & \cellbar{0.23}{0.97}{0.50}{0.27}{0.50} & \cellbar{0.09}{0.95}{0.69}{0.22}{0.31} & \cellbar{0.22}{0.95}{0.28}{0.50}{0.72} & \cellbar{0.18}{0.96}{0.43}{0.39}{0.57} & \cellbar{0.27}{0.92}{0.22}{0.51}{0.78} & \cellbar{0.16}{0.96}{0.51}{0.32}{0.49} & \cellbar{0.30}{0.83}{0.31}{0.39}{0.69} & \cellbar{0.24}{0.89}{0.46}{0.30}{0.54} & \cellbar{0.31}{0.84}{0.38}{0.31}{0.62} & \cellbar{0.15}{0.93}{0.30}{0.55}{0.70} & \cellbar{0.43}{0.79}{0.26}{0.31}{0.74} & \cellbar{0.04}{0.68}{0.70}{0.26}{0.30} & 0.89 \\
\textbf{21347} & \cellbar{0.05}{1.00}{0.88}{0.07}{0.12} & \cellbar{0.14}{0.99}{0.82}{0.04}{0.18} & \cellbar{0.05}{1.00}{0.84}{0.11}{0.16} & \cellbar{0.08}{0.99}{0.82}{0.09}{0.18} & \cellbar{0.16}{0.98}{0.74}{0.09}{0.26} & \cellbar{0.03}{1.00}{0.92}{0.05}{0.08} & \cellbar{0.07}{1.00}{0.93}{0.00}{0.07} & \cellbar{0.11}{1.00}{0.77}{0.12}{0.23} & \cellbar{0.04}{0.99}{0.80}{0.16}{0.20} & \cellbar{0.20}{0.96}{0.70}{0.09}{0.30} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.14}{0.92}{0.76}{0.11}{0.24} & \cellbar{0.01}{1.00}{0.95}{0.04}{0.05} & \cellbar{0.07}{1.00}{0.88}{0.05}{0.12} & \cellbar{0.05}{0.89}{0.89}{0.05}{0.11} & \cellbar{0.16}{0.97}{0.69}{0.15}{0.31} & \cellbar{0.01}{1.00}{0.96}{0.03}{0.04} & 0.98 \\
\textbf{30919} & \cellbar{0.20}{0.95}{0.42}{0.38}{0.58} & \cellbar{0.34}{0.77}{0.24}{0.42}{0.76} & \cellbar{0.28}{0.96}{0.36}{0.35}{0.64} & \cellbar{0.14}{0.95}{0.41}{0.46}{0.59} & \cellbar{0.27}{0.96}{0.49}{0.24}{0.51} & \cellbar{0.08}{0.87}{0.72}{0.20}{0.28} & \cellbar{0.23}{0.90}{0.59}{0.18}{0.41} & \cellbar{0.24}{0.92}{0.27}{0.49}{0.73} & \cellbar{0.30}{1.00}{0.35}{0.35}{0.65} & \cellbar{0.15}{0.97}{0.31}{0.54}{0.69} & \cellbar{0.07}{0.80}{0.86}{0.07}{0.14} & \cellbar{0.47}{0.93}{0.18}{0.35}{0.82} & \cellbar{0.41}{0.98}{0.46}{0.14}{0.54} & \cellbar{0.12}{0.94}{0.38}{0.50}{0.62} & \cellbar{0.23}{0.81}{0.16}{0.61}{0.84} & \cellbar{0.53}{0.96}{0.26}{0.22}{0.74} & \cellbar{0.16}{0.85}{0.68}{0.16}{0.32} & 0.91 \\
\textbf{34598} & \cellbar{0.14}{0.99}{0.78}{0.08}{0.22} & \cellbar{0.09}{0.94}{0.66}{0.24}{0.34} & \cellbar{0.14}{0.99}{0.69}{0.18}{0.31} & \cellbar{0.04}{0.96}{0.88}{0.08}{0.12} & \cellbar{0.12}{0.99}{0.82}{0.05}{0.18} & \cellbar{0.04}{0.98}{0.91}{0.05}{0.09} & \cellbar{0.07}{1.00}{0.91}{0.03}{0.09} & \cellbar{0.12}{0.98}{0.73}{0.15}{0.27} & \cellbar{0.07}{0.98}{0.72}{0.22}{0.28} & \cellbar{0.15}{0.98}{0.73}{0.12}{0.27} & \cellbar{0.03}{0.99}{0.96}{0.01}{0.04} & \cellbar{0.24}{0.97}{0.61}{0.15}{0.39} & \cellbar{0.09}{0.99}{0.86}{0.04}{0.14} & \cellbar{0.04}{0.96}{0.76}{0.20}{0.24} & \cellbar{0.01}{0.95}{0.85}{0.14}{0.15} & \cellbar{0.14}{0.91}{0.59}{0.27}{0.41} & \cellbar{0.00}{1.00}{0.96}{0.04}{0.04} & 0.98 \\
\textbf{41929} & \cellbar{0.08}{0.99}{0.77}{0.15}{0.23} & \cellbar{0.15}{1.00}{0.42}{0.43}{0.58} & \cellbar{0.15}{0.96}{0.70}{0.15}{0.30} & \cellbar{0.07}{1.00}{0.74}{0.19}{0.26} & \cellbar{0.19}{0.99}{0.69}{0.12}{0.31} & \cellbar{0.05}{0.85}{0.84}{0.11}{0.16} & \cellbar{0.15}{0.98}{0.78}{0.07}{0.22} & \cellbar{0.18}{0.94}{0.53}{0.30}{0.47} & \cellbar{0.15}{0.99}{0.57}{0.28}{0.43} & \cellbar{0.11}{0.92}{0.47}{0.42}{0.53} & \cellbar{0.04}{0.90}{0.96}{0.00}{0.04} & \cellbar{0.20}{0.90}{0.46}{0.34}{0.54} & \cellbar{0.35}{1.00}{0.59}{0.05}{0.41} & \cellbar{0.30}{0.95}{0.57}{0.14}{0.43} & \cellbar{0.12}{0.85}{0.64}{0.24}{0.36} & \cellbar{0.27}{0.86}{0.39}{0.34}{0.61} & \cellbar{0.05}{1.00}{0.88}{0.07}{0.12} & 0.95 \\
\textbf{47207} & \cellbar{0.14}{0.93}{0.58}{0.28}{0.42} & \cellbar{0.16}{0.76}{0.42}{0.42}{0.58} & \cellbar{0.23}{1.00}{0.54}{0.23}{0.46} & \cellbar{0.11}{0.94}{0.65}{0.24}{0.35} & \cellbar{0.26}{0.76}{0.53}{0.22}{0.47} & \cellbar{0.04}{0.95}{0.59}{0.36}{0.41} & \cellbar{0.11}{0.97}{0.73}{0.16}{0.27} & \cellbar{0.18}{0.94}{0.35}{0.47}{0.65} & \cellbar{0.12}{0.69}{0.34}{0.54}{0.66} & \cellbar{0.03}{0.81}{0.26}{0.72}{0.74} & \cellbar{0.04}{0.92}{0.54}{0.42}{0.46} & \cellbar{0.24}{0.90}{0.41}{0.35}{0.59} & \cellbar{0.31}{1.00}{0.46}{0.23}{0.54} & \cellbar{0.15}{0.98}{0.58}{0.27}{0.42} & \cellbar{0.19}{1.00}{0.26}{0.55}{0.74} & \cellbar{0.30}{0.82}{0.32}{0.38}{0.68} & \cellbar{0.15}{0.95}{0.84}{0.01}{0.16} & 0.90 \\
\textbf{48321} & \cellbar{0.22}{0.96}{0.51}{0.27}{0.49} & \cellbar{0.46}{0.53}{0.30}{0.24}{0.70} & \cellbar{0.18}{0.96}{0.55}{0.27}{0.45} & \cellbar{0.11}{0.95}{0.50}{0.39}{0.50} & \cellbar{0.16}{0.91}{0.57}{0.27}{0.43} & \cellbar{0.00}{0.92}{0.66}{0.34}{0.34} & \cellbar{0.15}{0.96}{0.72}{0.14}{0.28} & \cellbar{0.20}{0.95}{0.36}{0.43}{0.64} & \cellbar{0.32}{0.73}{0.58}{0.09}{0.42} & \cellbar{0.20}{1.00}{0.54}{0.26}{0.46} & \cellbar{0.08}{0.70}{0.85}{0.07}{0.15} & \cellbar{0.16}{0.95}{0.27}{0.57}{0.73} & \cellbar{0.23}{0.99}{0.72}{0.05}{0.28} & \cellbar{0.20}{0.83}{0.49}{0.31}{0.51} & \cellbar{0.05}{0.77}{0.22}{0.73}{0.78} & \cellbar{0.49}{0.93}{0.30}{0.22}{0.70} & \cellbar{0.04}{0.82}{0.81}{0.15}{0.19} & 0.87 \\
\textbf{49202} & \cellbar{0.14}{0.99}{0.80}{0.07}{0.20} & \cellbar{0.43}{0.82}{0.46}{0.11}{0.54} & \cellbar{0.16}{0.94}{0.58}{0.26}{0.42} & \cellbar{0.08}{0.97}{0.77}{0.15}{0.23} & \cellbar{0.22}{0.99}{0.57}{0.22}{0.43} & \cellbar{0.03}{0.82}{0.78}{0.19}{0.22} & \cellbar{0.11}{0.99}{0.84}{0.05}{0.16} & \cellbar{0.46}{0.94}{0.41}{0.14}{0.59} & \cellbar{0.23}{0.98}{0.70}{0.07}{0.30} & \cellbar{0.23}{0.98}{0.59}{0.18}{0.41} & \cellbar{0.04}{0.79}{0.95}{0.01}{0.05} & \cellbar{0.15}{0.96}{0.36}{0.49}{0.64} & \cellbar{0.08}{0.98}{0.82}{0.09}{0.18} & \cellbar{0.32}{0.90}{0.53}{0.15}{0.47} & \cellbar{0.12}{0.98}{0.65}{0.23}{0.35} & \cellbar{0.23}{0.82}{0.43}{0.34}{0.57} & \cellbar{0.07}{1.00}{0.82}{0.11}{0.18} & 0.93 \\
\textbf{51010} & \cellbar{0.04}{0.98}{0.89}{0.07}{0.11} & \cellbar{0.18}{0.92}{0.55}{0.27}{0.45} & \cellbar{0.18}{1.00}{0.66}{0.16}{0.34} & \cellbar{0.11}{0.99}{0.80}{0.09}{0.20} & \cellbar{0.38}{0.93}{0.51}{0.11}{0.49} & \cellbar{0.07}{0.79}{0.86}{0.07}{0.14} & \cellbar{0.22}{0.96}{0.76}{0.03}{0.24} & \cellbar{0.19}{0.95}{0.50}{0.31}{0.50} & \cellbar{0.16}{0.96}{0.70}{0.14}{0.30} & \cellbar{0.05}{0.96}{0.51}{0.43}{0.49} & \cellbar{0.03}{0.92}{0.95}{0.03}{0.05} & \cellbar{0.09}{0.98}{0.46}{0.45}{0.54} & \cellbar{0.09}{0.92}{0.64}{0.27}{0.36} & \cellbar{0.20}{0.98}{0.66}{0.14}{0.34} & \cellbar{0.07}{0.87}{0.66}{0.27}{0.34} & \cellbar{0.30}{0.69}{0.38}{0.32}{0.62} & \cellbar{0.04}{0.97}{0.91}{0.05}{0.09} & 0.93 \\
\textbf{54606} & \cellbar{0.11}{0.99}{0.70}{0.19}{0.30} & \cellbar{0.16}{0.97}{0.55}{0.28}{0.45} & \cellbar{0.14}{1.00}{0.76}{0.11}{0.24} & \cellbar{0.07}{1.00}{0.78}{0.15}{0.22} & \cellbar{0.31}{0.97}{0.64}{0.05}{0.36} & \cellbar{0.18}{1.00}{0.78}{0.04}{0.22} & \cellbar{0.09}{0.99}{0.86}{0.04}{0.14} & \cellbar{0.14}{0.91}{0.61}{0.26}{0.39} & \cellbar{0.16}{0.93}{0.59}{0.24}{0.41} & \cellbar{0.09}{0.88}{0.77}{0.14}{0.23} & \cellbar{0.05}{0.89}{0.95}{0.00}{0.05} & \cellbar{0.23}{0.95}{0.65}{0.12}{0.35} & \cellbar{0.04}{0.97}{0.81}{0.15}{0.19} & \cellbar{0.18}{0.99}{0.64}{0.19}{0.36} & \cellbar{0.03}{0.78}{0.77}{0.20}{0.23} & \cellbar{0.31}{0.83}{0.45}{0.24}{0.55} & \cellbar{0.01}{0.99}{0.95}{0.04}{0.05} & 0.94 \\
\textbf{58305} & \cellbar{0.11}{1.00}{0.76}{0.14}{0.24} & \cellbar{0.04}{1.00}{0.59}{0.36}{0.41} & \cellbar{0.11}{0.93}{0.77}{0.12}{0.23} & \cellbar{0.14}{0.96}{0.82}{0.04}{0.18} & \cellbar{0.01}{0.97}{0.77}{0.22}{0.23} & \cellbar{0.08}{0.95}{0.84}{0.08}{0.16} & \cellbar{0.07}{0.99}{0.82}{0.11}{0.18} & \cellbar{0.22}{0.89}{0.50}{0.28}{0.50} & \cellbar{0.07}{0.99}{0.72}{0.22}{0.28} & \cellbar{0.07}{0.89}{0.55}{0.38}{0.45} & \cellbar{0.03}{0.96}{0.95}{0.03}{0.05} & \cellbar{0.05}{0.87}{0.58}{0.36}{0.42} & \cellbar{0.03}{0.91}{0.89}{0.08}{0.11} & \cellbar{0.19}{0.97}{0.73}{0.08}{0.27} & \cellbar{0.08}{0.96}{0.69}{0.23}{0.31} & \cellbar{0.27}{0.66}{0.35}{0.38}{0.65} & \cellbar{0.05}{1.00}{0.92}{0.03}{0.08} & 0.93 \\
\textbf{60312} & \cellbar{0.22}{0.96}{0.51}{0.27}{0.49} & \cellbar{0.43}{0.81}{0.19}{0.38}{0.81} & \cellbar{0.36}{0.97}{0.34}{0.30}{0.66} & \cellbar{0.15}{0.90}{0.55}{0.30}{0.45} & \cellbar{0.54}{0.74}{0.26}{0.20}{0.74} & \cellbar{0.19}{0.64}{0.34}{0.47}{0.66} & \cellbar{0.12}{0.80}{0.51}{0.36}{0.49} & \cellbar{0.53}{0.82}{0.22}{0.26}{0.78} & \cellbar{0.59}{0.68}{0.24}{0.16}{0.76} & \cellbar{0.31}{0.62}{0.19}{0.50}{0.81} & \cellbar{0.05}{0.44}{0.85}{0.09}{0.15} & \cellbar{0.49}{0.94}{0.32}{0.19}{0.68} & \cellbar{0.32}{1.00}{0.49}{0.19}{0.51} & \cellbar{0.27}{0.98}{0.32}{0.41}{0.68} & \cellbar{0.24}{0.72}{0.22}{0.54}{0.78} & \cellbar{0.49}{0.83}{0.22}{0.30}{0.78} & \cellbar{0.09}{0.63}{0.80}{0.11}{0.20} & 0.79 \\
\textbf{62769} & \cellbar{0.24}{0.95}{0.47}{0.28}{0.53} & \cellbar{0.32}{0.89}{0.22}{0.46}{0.78} & \cellbar{0.42}{0.86}{0.32}{0.26}{0.68} & \cellbar{0.05}{0.96}{0.65}{0.30}{0.35} & \cellbar{0.50}{0.84}{0.26}{0.24}{0.74} & \cellbar{0.09}{0.91}{0.61}{0.30}{0.39} & \cellbar{0.11}{0.86}{0.57}{0.32}{0.43} & \cellbar{0.62}{0.69}{0.24}{0.14}{0.76} & \cellbar{0.24}{0.92}{0.55}{0.20}{0.45} & \cellbar{0.27}{0.62}{0.26}{0.47}{0.74} & \cellbar{0.05}{0.74}{0.80}{0.15}{0.20} & \cellbar{0.16}{0.68}{0.34}{0.50}{0.66} & \cellbar{0.14}{0.95}{0.74}{0.12}{0.26} & \cellbar{0.46}{0.95}{0.39}{0.15}{0.61} & \cellbar{0.30}{0.93}{0.36}{0.34}{0.64} & \cellbar{0.54}{0.74}{0.16}{0.30}{0.84} & \cellbar{0.04}{0.98}{0.86}{0.09}{0.14} & 0.85 \\
\textbf{63905} & \cellbar{0.26}{0.98}{0.58}{0.16}{0.42} & \cellbar{0.27}{0.76}{0.46}{0.27}{0.54} & \cellbar{0.26}{0.99}{0.45}{0.30}{0.55} & \cellbar{0.16}{0.94}{0.58}{0.26}{0.42} & \cellbar{0.46}{0.85}{0.45}{0.09}{0.55} & \cellbar{0.11}{0.82}{0.57}{0.32}{0.43} & \cellbar{0.26}{0.92}{0.64}{0.11}{0.36} & \cellbar{0.32}{0.90}{0.30}{0.38}{0.70} & \cellbar{0.16}{0.92}{0.47}{0.36}{0.53} & \cellbar{0.26}{0.73}{0.54}{0.20}{0.46} & \cellbar{0.03}{0.46}{0.65}{0.32}{0.35} & \cellbar{0.54}{0.92}{0.20}{0.26}{0.80} & \cellbar{0.22}{0.95}{0.51}{0.27}{0.49} & \cellbar{0.57}{0.90}{0.31}{0.12}{0.69} & \cellbar{0.07}{0.09}{0.23}{0.70}{0.77} & \cellbar{0.30}{0.90}{0.32}{0.38}{0.68} & \cellbar{0.14}{0.99}{0.77}{0.09}{0.23} & 0.82 \\
\bottomrule
\end{tabular}
}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!ht]
    \centering
\tikzstyle{mybox} = [draw=blue!50!white, fill=cyan!10!white, very thick,
    rectangle, rounded corners, inner sep=5pt, inner ysep=7pt]
\tikzstyle{fancytitle} =[fill=blue!50!white, text=white]
\tikzstyle{yellowbox} = [draw=red!50!white, fill=yellow!50, very thick,
    rectangle, rounded corners, inner sep=5pt, inner ysep=7pt]
\tikzstyle{fancytitlered} =[fill=red!70!white, text=white]
\tikzstyle{redbox} = [draw=red!50!white, fill=red!10, very thick,
    rectangle, rounded corners, inner sep=5pt, inner ysep=7pt]
\tikzstyle{greenbox} = [draw=red!50!white, fill=green!10, very thick,
    rectangle, rounded corners, inner sep=5pt, inner ysep=7pt]
\begin{tikzpicture}
\node [mybox] (box){%
    \begin{minipage}{0.60\textwidth}
        Answer the Question according to \fcolorbox{red!50!white}{yellow!50!white}{your values}.
        
        FYI, here is your trait. 
        ``Name: \fcolorbox{red!50}{red!10!white}{\texttt{Molly Lopez}}; 
        Gender: \fcolorbox{red!50}{red!10}{\texttt{female}};
        Job: \fcolorbox{red!50}{red!10!white}{\texttt{Energy manager}}; 
        MBTI: \fcolorbox{red!50}{red!10!white}{\texttt{ESTP}}".
        
        First write your Thought about the question, then Answer the question with 'yes' or 'no'.

        
        \textbf{Refer to the format of the following Examples.}

        \rule{0.03\textwidth}{0pt}
        \fcolorbox{red!50}{green!10}{
            \begin{minipage}{0.9\textwidth}
                [Example 1]:\\
            \textbf{Question:} Should I always be nice to others?\\
            \textbf{Thought:} Being nice to others may make me feel more accomplishment and live in a good mood.\\
            \textbf{Answer:} yes.
            
        [Example 2]:\\
        \textbf{Question:} Should I always be nice to others?\\
        \textbf{Thought:} Sometimes I have to be tough to protect myself so being nice is not always a good choice.\\
        \textbf{Answer}: no.
            \end{minipage}
        }
        
        \textbf{Now it is your turn.}\\
        Question: Should I always be a happy person?\\
        Thought:
    \end{minipage}
};
\node[fancytitle, right=10pt] at (box.north west) {Prompt to LLM};
\node[fancytitle, rounded corners] at ($(box.west)-(0.07,0)$) {$\clubsuit$};

\node [yellowbox] (ybox) at (7.7,3.76){%
    \begin{minipage}{0.3\textwidth}
        ``your values'': We choose one of the top-25 activated SAE features of these two tokens and enhanced 10 times in position.
    \end{minipage}
};
\node[fancytitlered, right=10pt] at ($(ybox.north west)+(0,0.1)$) {Steering position};

\node [redbox] (rbox) at (7.7,1.31){%
    \begin{minipage}{0.3\textwidth}
        %\texttt{Name}, \texttt{gender}, \texttt{job} and \texttt{MBTI type} form a brief description
        %of the identity $i\in\mathcal{I}$.
        \texttt{Name}, \texttt{gender}, \texttt{job} and \texttt{MBTI type} form a brief description
        of the role.
    \end{minipage}
};
\node[fancytitlered, right=10pt] at ($(rbox.north west)+(0,0.1)$) {Role Settings};

\node [greenbox] (gbox) at (7.7,-1.58){%
    \begin{minipage}{0.3\textwidth}
        To utilize in-context learning ability, two examples on 
        opposite opinions are given. Chain-of-Thought template is 
        given before any decision even in the example.
    \end{minipage}
};
\node[fancytitlered, right=10pt] at ($(gbox.north west)+(0,0.1)$) {In-context and CoT};

\node [mybox] (mbox) at (7.7,-4.3){%
    \begin{minipage}{0.3\textwidth}
        Thought: \texttt{[Thought]} \\ 
        Answer: \texttt{[yes / no]}
    \end{minipage}
};
\node[fancytitle, right=10pt] at ($(mbox.north west)+(0,0.1)$) {Output};
\node[fancytitle, rounded corners] at ($(mbox.east)$) {$\clubsuit$};
\end{tikzpicture}%
    
    \caption{\textbf{Experiment Design.}
    Single Q/A in dataset generation, the role-playing prompt template and SAE steering position.
    After run on all questions, 
    $S_T^{(f,\sigma)}$ can be calculated. In unsteered version, $\sigma=0$. In SAE steering version, $\sigma=10$. 
    Left: Input prompt to LLM. Right: Explanation of the prompt design and the output format.}
    \label{fig:prompt}
\end{figure*}

\begin{table*}
\centering
\caption{Value steering using SAE features for the Gemma-2B-IT model (above) and the Llama3-8B-IT model (below).}
\label{table: sae-steering-Gemma-2B-IT}
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1.5cm} *{10}{>{\centering\arraybackslash}m{1cm}}>{\centering\arraybackslash}m{1cm}}
\toprule
\rotatebox{90}{\textbf{SAE Feature}} & \rotatebox{90}{\textbf{Aesthetic}} & \rotatebox{90}{\textbf{Breadth of Interest}} & \rotatebox{90}{\textbf{Positive coping}} & \rotatebox{90}{\textbf{Religious}} & \rotatebox{90}{\textbf{Resilience}} & \rotatebox{90}{\textbf{Social}} & \rotatebox{90}{\textbf{Social Cynicism}} & \rotatebox{90}{\textbf{Theoretical}} & \rotatebox{90}{\textbf{Uncertainty Avoidance}} & \rotatebox{90}{\textbf{Understanding}} & \rotatebox{90}{\textbf{Mean Similarity}} \\
\midrule
\textbf{1312} & \cellbar{0.21}{0.96}{0.65}{0.14}{0.35} & \cellbar{0.00}{0.41}{0.29}{0.71}{0.71} & \cellbar{0.26}{0.67}{0.68}{0.06}{0.32} & \cellbar{0.55}{0.65}{0.41}{0.04}{0.59} & \cellbar{0.15}{0.90}{0.52}{0.33}{0.48} & \cellbar{0.04}{0.23}{0.91}{0.05}{0.09} & \cellbar{0.51}{0.10}{0.48}{0.01}{0.52} & \cellbar{0.34}{0.87}{0.60}{0.06}{0.40} & \cellbar{0.71}{0.94}{0.29}{0.00}{0.71} & \cellbar{0.01}{0.89}{0.76}{0.23}{0.24} & 0.66 \\
\textbf{1341} & \cellbar{0.27}{0.93}{0.56}{0.17}{0.44} & \cellbar{0.07}{0.91}{0.57}{0.36}{0.43} & \cellbar{0.39}{0.82}{0.56}{0.05}{0.44} & \cellbar{0.10}{0.99}{0.45}{0.46}{0.55} & \cellbar{0.39}{0.83}{0.58}{0.03}{0.42} & \cellbar{0.12}{0.94}{0.63}{0.25}{0.37} & \cellbar{0.00}{0.99}{0.90}{0.10}{0.10} & \cellbar{0.17}{0.97}{0.73}{0.10}{0.27} & \cellbar{0.18}{0.91}{0.68}{0.14}{0.32} & \cellbar{0.19}{0.66}{0.73}{0.08}{0.27} & 0.90 \\
\textbf{1975} & \cellbar{0.18}{0.81}{0.42}{0.41}{0.58} & \cellbar{0.05}{0.97}{0.71}{0.24}{0.29} & \cellbar{0.66}{0.91}{0.23}{0.11}{0.77} & \cellbar{0.18}{0.69}{0.48}{0.35}{0.52} & \cellbar{0.12}{0.71}{0.70}{0.18}{0.30} & \cellbar{0.02}{0.99}{0.82}{0.16}{0.18} & \cellbar{0.11}{0.80}{0.87}{0.02}{0.13} & \cellbar{0.01}{0.99}{0.80}{0.19}{0.20} & \cellbar{0.25}{0.99}{0.64}{0.11}{0.36} & \cellbar{0.03}{0.99}{0.68}{0.29}{0.32} & 0.89 \\
\textbf{2965} & \cellbar{0.02}{0.94}{0.71}{0.27}{0.29} & \cellbar{0.00}{0.87}{0.63}{0.37}{0.37} & \cellbar{0.23}{0.52}{0.73}{0.04}{0.27} & \cellbar{0.04}{0.99}{0.83}{0.13}{0.17} & \cellbar{0.01}{0.96}{0.76}{0.23}{0.24} & \cellbar{0.10}{0.99}{0.87}{0.03}{0.13} & \cellbar{0.01}{1.00}{0.85}{0.14}{0.15} & \cellbar{0.08}{1.00}{0.91}{0.01}{0.09} & \cellbar{0.19}{1.00}{0.64}{0.17}{0.36} & \cellbar{0.01}{0.99}{0.85}{0.14}{0.15} & 0.92 \\
\textbf{3183} & \cellbar{0.58}{0.66}{0.16}{0.26}{0.84} & \cellbar{0.16}{0.82}{0.35}{0.50}{0.65} & \cellbar{0.33}{0.87}{0.35}{0.33}{0.65} & \cellbar{0.76}{0.16}{0.16}{0.08}{0.84} & \cellbar{0.46}{0.55}{0.48}{0.07}{0.52} & \cellbar{0.28}{0.88}{0.27}{0.46}{0.73} & \cellbar{0.53}{0.83}{0.39}{0.08}{0.61} & \cellbar{0.68}{0.99}{0.20}{0.12}{0.80} & \cellbar{0.67}{0.94}{0.21}{0.12}{0.79} & \cellbar{0.18}{0.84}{0.34}{0.49}{0.66} & 0.75 \\
\textbf{3402} & \cellbar{0.16}{0.95}{0.63}{0.21}{0.37} & \cellbar{0.00}{0.69}{0.58}{0.42}{0.42} & \cellbar{0.26}{0.75}{0.68}{0.06}{0.32} & \cellbar{0.13}{0.97}{0.73}{0.14}{0.27} & \cellbar{0.03}{0.91}{0.62}{0.35}{0.38} & \cellbar{0.03}{0.99}{0.89}{0.08}{0.11} & \cellbar{0.06}{0.44}{0.90}{0.04}{0.10} & \cellbar{0.04}{1.00}{0.92}{0.04}{0.08} & \cellbar{0.21}{0.95}{0.60}{0.19}{0.40} & \cellbar{0.01}{0.82}{0.84}{0.15}{0.16} & 0.85 \\
\textbf{4752} & \cellbar{0.08}{0.64}{0.41}{0.51}{0.59} & \cellbar{0.20}{1.00}{0.53}{0.27}{0.47} & \cellbar{0.44}{0.87}{0.45}{0.12}{0.55} & \cellbar{0.07}{0.86}{0.58}{0.35}{0.42} & \cellbar{0.08}{1.00}{0.25}{0.67}{0.75} & \cellbar{0.03}{0.99}{0.81}{0.16}{0.19} & \cellbar{0.04}{0.93}{0.29}{0.67}{0.71} & \cellbar{0.21}{0.92}{0.61}{0.18}{0.39} & \cellbar{0.25}{0.91}{0.47}{0.29}{0.53} & \cellbar{0.36}{0.85}{0.55}{0.09}{0.45} & 0.90 \\
\textbf{6216} & \cellbar{0.06}{0.80}{0.50}{0.45}{0.50} & \cellbar{0.00}{0.49}{0.32}{0.68}{0.68} & \cellbar{0.27}{0.80}{0.65}{0.08}{0.35} & \cellbar{0.06}{0.99}{0.79}{0.15}{0.21} & \cellbar{0.18}{0.83}{0.50}{0.32}{0.50} & \cellbar{0.07}{0.99}{0.90}{0.03}{0.10} & \cellbar{0.34}{0.35}{0.66}{0.00}{0.34} & \cellbar{0.04}{1.00}{0.93}{0.03}{0.07} & \cellbar{0.29}{0.90}{0.60}{0.11}{0.40} & \cellbar{0.03}{0.99}{0.87}{0.10}{0.13} & 0.82 \\
\textbf{6619} & \cellbar{0.18}{0.82}{0.58}{0.24}{0.42} & \cellbar{0.02}{0.92}{0.68}{0.30}{0.32} & \cellbar{0.62}{0.99}{0.32}{0.06}{0.68} & \cellbar{0.22}{0.89}{0.40}{0.39}{0.60} & \cellbar{0.26}{0.60}{0.63}{0.11}{0.37} & \cellbar{0.05}{1.00}{0.90}{0.05}{0.10} & \cellbar{0.23}{0.58}{0.74}{0.03}{0.26} & \cellbar{0.02}{0.17}{0.74}{0.24}{0.26} & \cellbar{0.57}{0.76}{0.40}{0.03}{0.60} & \cellbar{0.09}{0.93}{0.71}{0.20}{0.29} & 0.77 \\
\textbf{7502} & \cellbar{0.02}{0.88}{0.63}{0.35}{0.37} & \cellbar{0.00}{0.89}{0.64}{0.36}{0.36} & \cellbar{0.24}{0.92}{0.67}{0.09}{0.33} & \cellbar{0.04}{0.99}{0.84}{0.12}{0.16} & \cellbar{0.04}{0.93}{0.66}{0.30}{0.34} & \cellbar{0.03}{1.00}{0.86}{0.11}{0.14} & \cellbar{0.01}{0.44}{0.90}{0.09}{0.10} & \cellbar{0.03}{1.00}{0.94}{0.03}{0.06} & \cellbar{0.22}{0.97}{0.64}{0.14}{0.36} & \cellbar{0.06}{0.98}{0.87}{0.07}{0.13} & 0.90 \\
\textbf{10096} & \cellbar{0.27}{0.73}{0.36}{0.38}{0.64} & \cellbar{0.41}{0.97}{0.45}{0.15}{0.55} & \cellbar{0.07}{0.81}{0.65}{0.28}{0.35} & \cellbar{0.27}{0.63}{0.44}{0.30}{0.56} & \cellbar{0.25}{0.53}{0.51}{0.24}{0.49} & \cellbar{0.27}{0.97}{0.44}{0.30}{0.56} & \cellbar{0.13}{0.74}{0.86}{0.01}{0.14} & \cellbar{0.62}{0.88}{0.38}{0.00}{0.62} & \cellbar{0.27}{0.81}{0.44}{0.30}{0.56} & \cellbar{0.41}{0.83}{0.50}{0.10}{0.50} & 0.79 \\
\textbf{10605} & \cellbar{0.13}{0.99}{0.35}{0.52}{0.65} & \cellbar{0.02}{0.83}{0.56}{0.42}{0.44} & \cellbar{0.32}{0.79}{0.66}{0.02}{0.34} & \cellbar{0.20}{0.72}{0.43}{0.38}{0.57} & \cellbar{0.11}{0.96}{0.36}{0.53}{0.64} & \cellbar{0.04}{0.98}{0.82}{0.14}{0.18} & \cellbar{0.03}{0.99}{0.80}{0.17}{0.20} & \cellbar{0.36}{0.78}{0.61}{0.03}{0.39} & \cellbar{0.42}{0.96}{0.42}{0.17}{0.58} & \cellbar{0.10}{0.56}{0.74}{0.16}{0.26} & 0.86 \\
\textbf{11712} & \cellbar{0.23}{0.98}{0.63}{0.14}{0.37} & \cellbar{0.01}{0.96}{0.93}{0.06}{0.07} & \cellbar{0.15}{0.93}{0.78}{0.07}{0.22} & \cellbar{0.03}{0.95}{0.78}{0.19}{0.22} & \cellbar{0.09}{0.87}{0.54}{0.37}{0.46} & \cellbar{0.08}{1.00}{0.89}{0.03}{0.11} & \cellbar{0.01}{0.67}{0.98}{0.01}{0.02} & \cellbar{0.12}{0.88}{0.71}{0.17}{0.29} & \cellbar{0.14}{0.78}{0.73}{0.13}{0.27} & \cellbar{0.09}{0.78}{0.80}{0.11}{0.20} & 0.88 \\
\textbf{14049} & \cellbar{0.10}{0.60}{0.34}{0.56}{0.66} & \cellbar{0.02}{0.99}{0.57}{0.41}{0.43} & \cellbar{0.32}{0.74}{0.56}{0.12}{0.44} & \cellbar{0.21}{0.89}{0.50}{0.29}{0.50} & \cellbar{0.12}{0.65}{0.36}{0.52}{0.64} & \cellbar{0.16}{0.99}{0.72}{0.12}{0.28} & \cellbar{0.44}{0.84}{0.54}{0.02}{0.46} & \cellbar{0.38}{0.71}{0.55}{0.07}{0.45} & \cellbar{0.54}{1.00}{0.38}{0.08}{0.62} & \cellbar{0.13}{0.96}{0.60}{0.27}{0.40} & 0.84 \\
\textbf{14185} & \cellbar{0.29}{0.96}{0.51}{0.20}{0.49} & \cellbar{0.08}{0.98}{0.74}{0.18}{0.26} & \cellbar{0.38}{0.79}{0.58}{0.04}{0.42} & \cellbar{0.12}{0.98}{0.57}{0.31}{0.43} & \cellbar{0.09}{0.97}{0.66}{0.25}{0.34} & \cellbar{0.04}{1.00}{0.77}{0.19}{0.23} & \cellbar{0.06}{0.92}{0.77}{0.17}{0.23} & \cellbar{0.19}{0.95}{0.78}{0.03}{0.22} & \cellbar{0.28}{0.75}{0.65}{0.07}{0.35} & \cellbar{0.04}{0.63}{0.75}{0.21}{0.25} & 0.89 \\
\midrule
Noise Ratio:& 0.13&0.05&0.09&0.12&0.10&0.08&0.02&0.06&0.13&0.07 \\
\bottomrule
\midrule
\textbf{4305} & \cellbar{0.45}{0.66}{0.20}{0.35}{0.80} & \cellbar{0.16}{0.93}{0.54}{0.30}{0.46} & \cellbar{0.34}{0.88}{0.31}{0.35}{0.69} & \cellbar{0.16}{0.77}{0.19}{0.65}{0.81} & \cellbar{0.03}{0.64}{0.49}{0.49}{0.51} & \cellbar{0.16}{1.00}{0.24}{0.59}{0.76} & \cellbar{0.08}{0.98}{0.34}{0.58}{0.66} & \cellbar{0.15}{0.52}{0.22}{0.64}{0.78} & \cellbar{0.39}{0.52}{0.32}{0.28}{0.68} & \cellbar{0.11}{0.21}{0.89}{0.00}{0.11} & 0.71 \\
\textbf{8035} & \cellbar{0.03}{0.97}{0.81}{0.16}{0.19} & \cellbar{0.03}{0.98}{0.93}{0.04}{0.07} & \cellbar{0.05}{1.00}{0.91}{0.04}{0.09} & \cellbar{0.08}{1.00}{0.89}{0.03}{0.11} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.01}{0.98}{0.89}{0.09}{0.11} & \cellbar{0.08}{1.00}{0.88}{0.04}{0.12} & \cellbar{0.03}{0.92}{0.86}{0.11}{0.14} & \cellbar{0.05}{0.96}{0.73}{0.22}{0.27} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & 0.98 \\
\textbf{8546} & \cellbar{0.20}{0.88}{0.47}{0.32}{0.53} & \cellbar{0.14}{0.99}{0.66}{0.20}{0.34} & \cellbar{0.27}{0.98}{0.57}{0.16}{0.43} & \cellbar{0.16}{1.00}{0.50}{0.34}{0.50} & \cellbar{0.03}{0.96}{0.92}{0.05}{0.08} & \cellbar{0.12}{0.88}{0.50}{0.38}{0.50} & \cellbar{0.27}{0.96}{0.58}{0.15}{0.42} & \cellbar{0.05}{0.84}{0.59}{0.35}{0.41} & \cellbar{0.53}{0.57}{0.27}{0.20}{0.73} & \cellbar{0.07}{1.00}{0.89}{0.04}{0.11} & 0.91 \\
\textbf{9332} & \cellbar{0.43}{0.97}{0.15}{0.42}{0.85} & \cellbar{0.09}{0.49}{0.27}{0.64}{0.73} & \cellbar{0.45}{0.77}{0.34}{0.22}{0.66} & \cellbar{0.51}{0.98}{0.28}{0.20}{0.72} & \cellbar{0.30}{0.80}{0.49}{0.22}{0.51} & \cellbar{0.28}{0.79}{0.22}{0.50}{0.78} & \cellbar{0.78}{0.89}{0.12}{0.09}{0.88} & \cellbar{0.41}{0.84}{0.19}{0.41}{0.81} & \cellbar{0.61}{0.70}{0.16}{0.23}{0.84} & \cellbar{0.12}{0.99}{0.46}{0.42}{0.54} & 0.82 \\
\textbf{12477} & \cellbar{0.07}{1.00}{0.81}{0.12}{0.19} & \cellbar{0.05}{1.00}{0.91}{0.04}{0.09} & \cellbar{0.07}{0.99}{0.89}{0.04}{0.11} & \cellbar{0.07}{1.00}{0.81}{0.12}{0.19} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.07}{0.96}{0.89}{0.04}{0.11} & \cellbar{0.07}{1.00}{0.89}{0.04}{0.11} & \cellbar{0.04}{1.00}{0.86}{0.09}{0.14} & \cellbar{0.04}{0.96}{0.78}{0.18}{0.22} & \cellbar{0.01}{1.00}{0.99}{0.00}{0.01} & 0.99 \\
\textbf{21347} & \cellbar{0.14}{0.99}{0.82}{0.04}{0.18} & \cellbar{0.08}{0.99}{0.82}{0.09}{0.18} & \cellbar{0.04}{0.99}{0.80}{0.16}{0.20} & \cellbar{0.20}{0.96}{0.70}{0.09}{0.30} & \cellbar{0.00}{1.00}{0.99}{0.01}{0.01} & \cellbar{0.14}{0.92}{0.76}{0.11}{0.24} & \cellbar{0.07}{1.00}{0.88}{0.05}{0.12} & \cellbar{0.05}{0.89}{0.89}{0.05}{0.11} & \cellbar{0.16}{0.97}{0.69}{0.15}{0.31} & \cellbar{0.01}{1.00}{0.96}{0.03}{0.04} & 0.97 \\
\textbf{30919} & \cellbar{0.34}{0.77}{0.24}{0.42}{0.76} & \cellbar{0.14}{0.95}{0.41}{0.46}{0.59} & \cellbar{0.30}{1.00}{0.35}{0.35}{0.65} & \cellbar{0.15}{0.97}{0.31}{0.54}{0.69} & \cellbar{0.07}{0.80}{0.86}{0.07}{0.14} & \cellbar{0.47}{0.93}{0.18}{0.35}{0.82} & \cellbar{0.12}{0.94}{0.38}{0.50}{0.62} & \cellbar{0.23}{0.81}{0.16}{0.61}{0.84} & \cellbar{0.53}{0.96}{0.26}{0.22}{0.74} & \cellbar{0.16}{0.85}{0.68}{0.16}{0.32} & 0.90 \\
\textbf{34598} & \cellbar{0.09}{0.94}{0.66}{0.24}{0.34} & \cellbar{0.04}{0.96}{0.88}{0.08}{0.12} & \cellbar{0.07}{0.98}{0.72}{0.22}{0.28} & \cellbar{0.15}{0.98}{0.73}{0.12}{0.27} & \cellbar{0.03}{0.99}{0.96}{0.01}{0.04} & \cellbar{0.24}{0.97}{0.61}{0.15}{0.39} & \cellbar{0.04}{0.96}{0.76}{0.20}{0.24} & \cellbar{0.01}{0.95}{0.85}{0.14}{0.15} & \cellbar{0.14}{0.91}{0.59}{0.27}{0.41} & \cellbar{0.00}{1.00}{0.96}{0.04}{0.04} & 0.96 \\
\textbf{47207} & \cellbar{0.16}{0.76}{0.42}{0.42}{0.58} & \cellbar{0.11}{0.94}{0.65}{0.24}{0.35} & \cellbar{0.12}{0.69}{0.34}{0.54}{0.66} & \cellbar{0.03}{0.81}{0.26}{0.72}{0.74} & \cellbar{0.04}{0.92}{0.54}{0.42}{0.46} & \cellbar{0.24}{0.90}{0.41}{0.35}{0.59} & \cellbar{0.15}{0.98}{0.58}{0.27}{0.42} & \cellbar{0.19}{1.00}{0.26}{0.55}{0.74} & \cellbar{0.30}{0.82}{0.32}{0.38}{0.68} & \cellbar{0.15}{0.95}{0.84}{0.01}{0.16} & 0.88 \\
\textbf{51010} & \cellbar{0.18}{0.92}{0.55}{0.27}{0.45} & \cellbar{0.11}{0.99}{0.80}{0.09}{0.20} & \cellbar{0.16}{0.96}{0.70}{0.14}{0.30} & \cellbar{0.05}{0.96}{0.51}{0.43}{0.49} & \cellbar{0.03}{0.92}{0.95}{0.03}{0.05} & \cellbar{0.09}{0.98}{0.46}{0.45}{0.54} & \cellbar{0.20}{0.98}{0.66}{0.14}{0.34} & \cellbar{0.07}{0.87}{0.66}{0.27}{0.34} & \cellbar{0.30}{0.69}{0.38}{0.32}{0.62} & \cellbar{0.04}{0.97}{0.91}{0.05}{0.09} & 0.92 \\
\textbf{54606} & \cellbar{0.16}{0.97}{0.55}{0.28}{0.45} & \cellbar{0.07}{1.00}{0.78}{0.15}{0.22} & \cellbar{0.16}{0.93}{0.59}{0.24}{0.41} & \cellbar{0.09}{0.88}{0.77}{0.14}{0.23} & \cellbar{0.05}{0.89}{0.95}{0.00}{0.05} & \cellbar{0.23}{0.95}{0.65}{0.12}{0.35} & \cellbar{0.18}{0.99}{0.64}{0.19}{0.36} & \cellbar{0.03}{0.78}{0.77}{0.20}{0.23} & \cellbar{0.31}{0.83}{0.45}{0.24}{0.55} & \cellbar{0.01}{0.99}{0.95}{0.04}{0.05} & 0.92 \\
\textbf{62769} & \cellbar{0.32}{0.89}{0.22}{0.46}{0.78} & \cellbar{0.05}{0.96}{0.65}{0.30}{0.35} & \cellbar{0.24}{0.92}{0.55}{0.20}{0.45} & \cellbar{0.27}{0.62}{0.26}{0.47}{0.74} & \cellbar{0.05}{0.74}{0.80}{0.15}{0.20} & \cellbar{0.16}{0.68}{0.34}{0.50}{0.66} & \cellbar{0.46}{0.95}{0.39}{0.15}{0.61} & \cellbar{0.30}{0.93}{0.36}{0.34}{0.64} & \cellbar{0.54}{0.74}{0.16}{0.30}{0.84} & \cellbar{0.04}{0.98}{0.86}{0.09}{0.14} & 0.84 \\
\midrule
Noise Ratio:& 0.15&0.09&0.15&0.12&0.04&0.13&0.10&0.11&0.19&0.04 \\
\bottomrule
\end{tabular}
}
\end{table*}

